Full abstraction for fair testing in CCS (expanded version)

In previous work with Pous, we defined a semantics for CCS which may both be viewed as an innocent form of presheaf semantics and as a concurrent form of game semantics. We define in this setting an analogue of fair testing equivalence, which we prove fully abstract w.r.t. standard fair testing equivalence. The proof relies on a new algebraic notion called playground, which represents the `rule of the game'. From any playground, we derive two languages equipped with labelled transition systems, as well as a strong, functional bisimulation between them.

==> pgflibraryarrows.new.code.tex <==
% alternative * arrow
\pgfarrowsdeclare{* new}{* new}
{
  \ifdim\pgfgetarrowoptions{* new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=5.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=1.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{* new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsleftextend{+-0.5\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \ifdim\pgfgetarrowoptions{* new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%  
    \pgfpathcircle{\pgfqpoint{-3\pgfutil@tempdima}{0pt}}{+4.5\pgfutil@tempdima}
    \pgfusepathqfillstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{* new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 2%
    \pgfpathcircle{\pgfqpoint{\pgfutil@tempdima}{0pt}}{\pgfutil@tempdima}
    \pgfusepathqfillstroke
  \fi
}

% alternative round bracket arrow
\pgfarrowsdeclare{( new}{) new}
{
  \ifdim\pgfgetarrowoptions{) new}<0pt%
    \pgfutil@tempdima=2pt%
    \advance\pgfutil@tempdima by1.5\pgflinewidth%
    \pgfutil@tempdimb=0.0625\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
    \pgfutil@tempdimb=0.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{) new}%
    \pgfutil@tempdima=0.28125\pgfutil@tempdima%
    \advance\pgfutil@tempdima by 0.21875\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.5\pgflinewidth}  
  \fi
}
{
  \ifdim\pgfgetarrowoptions{) new}<0pt%
    \pgfutil@tempdima=2pt%
    \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{) new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 2%
    \pgftransformxshift{-0.0625\pgfutil@tempdima}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{-.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{.25\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{.25\pgfutil@tempdima}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-.5\pgfutil@tempdima}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative round bracket reversed arrow
\pgfarrowsdeclarereversed{) new}{( new}{( new}{) new}

% alternative square bracket arrow. Use with {[ new}-{] new}
\pgfarrowsdeclare{[ new}{] new}
{
  \pgfutil@tempdima=1pt%
  \advance\pgfutil@tempdima by1.25\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdima}
  \pgfarrowsrightextend{+.5\pgflinewidth}
}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfutil@tempdimb=\pgfutil@tempdima%
  \advance\pgfutil@tempdimb by\pgflinewidth%
  \unless\ifdim\pgfgetarrowoptions{] new}<0pt%
    \pgfutil@tempdima=\pgfgetarrowoptions{] new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 2%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{-.5\pgfutil@tempdimb}{-1\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{-1\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-.5\pgfutil@tempdimb}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative square bracket reversed arrow. Use with {] new}-{[ new}
\pgfarrowsdeclarereversed{] new}{[ new}{[ new}{] new}

% alternative | arrow
\pgfarrowsdeclare{| new}{| new}
{
  \pgfarrowsleftextend{+-0.25\pgflinewidth}
  \pgfarrowsrightextend{+.75\pgflinewidth}
}
{
  \ifdim\pgfgetarrowoptions{| new}<0pt%
    \pgfutil@tempdima=2pt%
    \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{| new}%
    \advance\pgfutil@tempdima by -\pgflinewidth% due to rect line cap
    \divide\pgfutil@tempdima by 2%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetrectcap
  \pgfpathmoveto{\pgfqpoint{0.25\pgflinewidth}{-\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.25\pgflinewidth}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative angle 45 arrow
\pgfarrowsdeclare{angle 45 new}{angle 45 new}
{
  \ifdim\pgfgetarrowoptions{angle 45 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=8.705\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by1.28\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 45 new}%
    \advance\pgfutil@tempdima by -1.30656\pgflinewidth% 0.5*cosec(\alpha/2)
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+1.30656\pgflinewidth}  
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{angle 45 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 45 new}%
    \advance\pgfutil@tempdima by -1.80656\pgflinewidth% -(1.30656+0.5)
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(22.5)} 
    \pgfpathmoveto{\pgfqpointpolar{157.5}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-157.5}{\pgfutil@tempdima}}
    \pgfusepathqstroke
  \fi
}

% alternative angle 45 reversed arrow
\pgfarrowsdeclarereversed{angle 45 new reversed}{angle 45 new reversed}{angle 45 new}{angle 45 new}

% alternative angle 60 arrow
\pgfarrowsdeclare{angle 60 new}{angle 60 new}
{
  \ifdim\pgfgetarrowoptions{angle 60 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=7.29\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 60 new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgflinewidth}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{angle 60 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 60 new}%
    \advance\pgfutil@tempdima by -1.5\pgflinewidth% -(1+0.5)
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(30)}    
    \pgfpathmoveto{\pgfqpointpolar{150}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-150}{\pgfutil@tempdima}}
    \pgfusepathqstroke
  \fi
}

% alternative angle 60 reversed arrow
\pgfarrowsdeclarereversed{angle 60 new reversed}{angle 60 new reversed}{angle 60 new}{angle 60 new}

% alternative angle 90 arrow
\pgfarrowsdeclare{angle 90 new}{angle 90 new}
{
  \ifdim\pgfgetarrowoptions{angle 90 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=5.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.707\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 90 new}%
    \advance\pgfutil@tempdima by -0.70711\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.70711\pgflinewidth}  
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{angle 90 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfqpoint{-5.5\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{-5.5\pgfutil@tempdima}{6\pgfutil@tempdima}}
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 90 new}%
    \advance\pgfutil@tempdima by -1.20711\pgflinewidth% -(0.70711+0.5)
    \pgfpathmoveto{\pgfqpoint{-\pgfutil@tempdima}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}
    \pgfusepathqstroke
  \fi    
}

% alternative angle 90 reversed arrow
\pgfarrowsdeclarereversed{angle 90 new reversed}{angle 90 new reversed}{angle 90 new}{angle 90 new}

% original butt cap arrow (just for completeness)
\pgfarrowsdeclare{butt cap new}{butt cap new}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+.5\pgflinewidth}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}

% alternative diamond arrow
\pgfarrowsdeclare{diamond new}{diamond new}
{
  \ifdim\pgfgetarrowoptions{diamond new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
    \pgfutil@tempdimb=13\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=1\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{diamond new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsleftextend{+-0.5\pgflinewidth}% due to the round cap
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{diamond new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{diamond new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 14%
    \pgftransformxshift{13\pgfutil@tempdima}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{1\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-6\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-13\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-6\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

% original fast cap arrow (just for completeness)
\pgfarrowsdeclare{fast cap new}{fast cap new}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+2\pgflinewidth}
}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfqpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}

% original fast cap reversed arrow (just for completeness)
\pgfarrowsdeclare{fast cap new reversed}{fast cap new reversed}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+2\pgflinewidth}
}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfqpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}

% alternative hooks arrow
\pgfarrowsdeclare{hooks new}{hooks new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \ifdim\pgfgetarrowoptions{hooks new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{hooks new}%
    \pgfutil@tempdima=0.3125\pgfutil@tempdima%
    \advance\pgfutil@tempdima by 0.1875\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}%
  \fi
}
{
  \ifdim\pgfgetarrowoptions{hooks new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{hooks new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 12%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{1.665\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{3\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.75\pgfutil@tempdima}{4.665\pgfutil@tempdima}}
    {\pgfqpoint{2.415\pgfutil@tempdima}{6\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathmoveto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{-1.665\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{-3\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.75\pgfutil@tempdima}{-4.665\pgfutil@tempdima}}
    {\pgfqpoint{2.415\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}

% alternative hooks reversed arrow
\pgfarrowsdeclarereversed{hooks new reversed}{hooks new reversed}{hooks new}{hooks new}

% original implies arrow (just for completeness)
\pgfarrowsdeclare{implies new}{implies new}
{
  \pgfmathsetlength{\pgfutil@tempdima}{.25\pgflinewidth+.25*\pgfinnerlinewidth}%
  \pgfmathsetlength{\pgfutil@tempdimb}{.5\pgflinewidth-.5*\pgfinnerlinewidth}%
  \pgfarrowsrightextend{2\pgfutil@tempdima+.5\pgfutil@tempdimb}
  \pgfarrowsleftextend{1.3\pgfutil@tempdima+.5\pgfutil@tempdimb}
}
{
  \pgfmathsetlength{\pgfutil@tempdima}{.25\pgflinewidth+.25*\pgfinnerlinewidth}%
  \pgfmathsetlength{\pgfutil@tempdimb}{.5\pgflinewidth-.5*\pgfinnerlinewidth}%
  \pgfsetlinewidth{\pgfutil@tempdimb}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{-1.4\pgfutil@tempdima}{2.65\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-0.75\pgfutil@tempdima}{1.25\pgfutil@tempdima}}
  {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
  {\pgfpoint{2\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
  {\pgfpoint{-.75\pgfutil@tempdima}{-1.25\pgfutil@tempdima}}
  {\pgfpoint{-1.4\pgfutil@tempdima}{-2.65\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative latex arrow
\pgfarrowsdeclare{latex new}{latex new}
{
  \ifdim\pgfgetarrowoptions{latex new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \pgfutil@tempdimb=\pgflinewidth%
    \ifdim\pgfinnerlinewidth>0pt%
      \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
    \fi
    \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
    \pgfarrowsleftextend{+-1\pgfutil@tempdima}
    \pgfarrowsrightextend{+9\pgfutil@tempdima}
  \else
     \pgfutil@tempdima=\pgfgetarrowoptions{latex new}%
     \advance\pgfutil@tempdima by -0.5pt% to minimize the arrow shaft
     \pgfarrowsleftextend{+-0.5pt}
     \pgfarrowsrightextend{\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{latex new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \pgfutil@tempdimb=\pgflinewidth%
    \ifdim\pgfinnerlinewidth>0pt%
      \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
    \fi
    \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{latex new}%
    \divide\pgfutil@tempdima by 10%
    \pgfutil@tempdimb=\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.5pt%
    \pgftransformxshift{\pgfutil@tempdimb}% to minimize the arrow shaft
  \fi
  \pgfpathmoveto{\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
    {\pgfqpoint{6.3333\pgfutil@tempdima}{.5\pgfutil@tempdima}}
    {\pgfqpoint{2\pgfutil@tempdima}{2\pgfutil@tempdima}}
    {\pgfqpoint{-1\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-1\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2\pgfutil@tempdima}{-2\pgfutil@tempdima}}
    {\pgfqpoint{6.3333\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfusepathqfill
}

% alternative latex reversed arrow
\pgfarrowsdeclarereversed{latex new reversed}{latex new reversed}{latex new}{latex new}

% alternative latex' arrow
\pgfarrowsdeclare{latex' new}{latex' new}
{
  \ifdim\pgfgetarrowoptions{latex' new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
    \pgfarrowsleftextend{+-4\pgfutil@tempdima}
    \pgfarrowsrightextend{+6\pgfutil@tempdima}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{latex' new}%
    \pgfutil@tempdimb=0.8125\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.5pt%
    \advance\pgfutil@tempdima by -\pgfutil@tempdimb%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}% to minimize the arrow shaft
    \pgfarrowsrightextend{+\pgfutil@tempdimb}%
  \fi
}
{
  \ifdim\pgfgetarrowoptions{latex' new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{latex' new}%
    \divide\pgfutil@tempdima by 10%
    \pgfutil@tempdimb=2.125\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.5pt%
    \pgftransformxshift{\pgfutil@tempdimb}% to minimize the arrow shaft
  \fi
  \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-1\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
    {\pgfqpoint{-4\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-1.5\pgfutil@tempdima}{1\pgfutil@tempdima}}
    {\pgfqpoint{-1.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
    {\pgfqpoint{-4\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-1\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
    {\pgfqpoint{3.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfusepathqfill
}

% alternative latex' reversed arrow
\pgfarrowsdeclarereversed{latex' new reversed}{latex' new reversed}{latex' new}{latex' new}

% alternative left hook arrow
\pgfarrowsdeclare{left hook new}{left hook new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \ifdim\pgfgetarrowoptions{left hook new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left hook new}%
    \pgfutil@tempdima=0.3125\pgfutil@tempdima%
    \advance\pgfutil@tempdima by 0.1875\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{left hook new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left hook new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 12%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{1.665\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{3\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.75\pgfutil@tempdima}{4.665\pgfutil@tempdima}}
    {\pgfqpoint{2.415\pgfutil@tempdima}{6\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}

% alternative left hook reversed arrow
\pgfarrowsdeclarereversed{left hook new reversed}{left hook new reversed}{left hook new}{left hook new}

% alternative left to arrow
\pgfarrowsdeclare{left to new}{left to new}
{
  \ifdim\pgfgetarrowoptions{left to new}<0pt%
    \pgfutil@tempdima=-0.84pt%
    \advance\pgfutil@tempdima by-1.3\pgflinewidth%
    \pgfutil@tempdimb=0.21pt%
    \advance\pgfutil@tempdimb by.625\pgflinewidth%
    \pgfarrowsleftextend{+\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% arbitrary value (2*0.5*0.8\pgflinewidth)
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.8\pgflinewidth}%
  \fi
}
{
  \ifdim\pgfgetarrowoptions{left to new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
    \pgfutil@tempdimb=0pt%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%
    \multiply\pgfutil@tempdima by 4%
    \pgfutil@tempdimb=0.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.4\pgflinewidth% arbitrary value (0.5*0.8\pgflinewidth)
    \pgftransformxshift{-\pgfutil@tempdimb}
  \fi  
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{0.25\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
    {\pgfqpoint{0.55\pgfutil@tempdima}{-0.125\pgflinewidth}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{-0.125\pgflinewidth}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{-0.125\pgflinewidth}} 
  \pgfpathlineto{\pgfqpoint{\pgfutil@tempdimb}{-0.125\pgflinewidth}}
  \pgfusepathqstroke
}

% alternative left to reversed arrow
\pgfarrowsdeclare{left to new reversed}{left to new reversed}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \ifdim\pgfgetarrowoptions{left to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth% 
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.9\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new reversed}%
    \advance\pgfutil@tempdima by 0.1\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{left to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new reversed}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{4\pgfutil@tempdima}}
    \pgfpathcurveto
      {\pgfqpoint{3.5\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
      {\pgfqpoint{0.75\pgfutil@tempdima}{0.25\pgfutil@tempdima}}
      {\pgfqpoint{0pt}{0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{4\pgfutil@tempdima}}
    \pgfpathcurveto
      {\pgfqpoint{3.5\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
      {\pgfqpoint{0.75\pgfutil@tempdima}{0.25\pgfutil@tempdima}}
      {\pgfqpoint{0pt}{-0.125\pgflinewidth}}
  }
  \pgfusepathqstroke
}

% alternative o arrow
\pgfarrowsdeclare{o new}{o new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \ifdim\pgfgetarrowoptions{o new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=9\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{o new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{ 
  \ifdim\pgfgetarrowoptions{o new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{o new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 9%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfpathcircle{\pgfqpoint{4.5\pgfutil@tempdima}{0pt}}{4.5\pgfutil@tempdima}%
  \pgfusepathqstroke
}

% alternative open diamond arrow
\pgfarrowsdeclare{open diamond new}{open diamond new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}% due to the round cap
  \ifdim\pgfgetarrowoptions{open diamond new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
    \pgfutil@tempdimb=14\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open diamond new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{open diamond new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open diamond new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 14%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{14\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{7\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{7\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}

% alternative open square arrow
\pgfarrowsdeclare{open square new}{open square new}
{
  \ifdim\pgfgetarrowoptions{open square new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
    \advance\pgfutil@tempdima by7\pgfutil@tempdima%
    \advance\pgfutil@tempdima by.5\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open square new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
  \fi
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfarrowsrightextend{+\pgfutil@tempdima}
}
{
  \ifdim\pgfgetarrowoptions{open square new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open square new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 8%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{8\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{8\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}

% alternative open triangle 45 arrow
\pgfarrowsdeclare{open triangle 45 new}{open triangle 45 new}
{
  \ifdim\pgfgetarrowoptions{open triangle 45 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=9.205\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by1.28\pgflinewidth%
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 45 new}%
    \advance\pgfutil@tempdimb by -0.5\pgflinewidth%
  \fi
    \pgfarrowsleftextend{+-.5\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin  
  \ifdim\pgfgetarrowoptions{open triangle 45 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 45 new}%
    \advance\pgfutil@tempdima by -1.80656\pgflinewidth% -(1.30656+0.5)
    \pgftransformxshift{\pgfutil@tempdima}
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(22.5)}    
    \pgfpathmoveto{\pgfqpointpolar{157.5}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-157.5}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi    
}

% alternative open triangle 45 reversed arrow
\pgfarrowsdeclare{open triangle 45 new reversed}{open triangle 45 new reversed}
{
  \ifdim\pgfgetarrowoptions{open triangle 45 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfarrowsleftextend{+-1.28\pgflinewidth}
    \pgfutil@tempdimb=9.205\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \else
    \pgfarrowsleftextend{+-1.30656\pgflinewidth}%
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 45 new reversed}%
    \advance\pgfutil@tempdimb by -1.30656\pgflinewidth%
  \fi
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 45 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfqpointpolar{23}{10\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-23}{10\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 45 new reversed}%
    \advance\pgfutil@tempdima by -1.80656\pgflinewidth% -(1.30656+0.5)
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(22.5)}    
    \pgfpathmoveto{\pgfqpointpolar{22.5}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-22.5}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi  
}

% alternative open triangle 60 arrow
\pgfarrowsdeclare{open triangle 60 new}{open triangle 60 new}
{
  \ifdim\pgfgetarrowoptions{open triangle 60 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=7.794\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by\pgflinewidth%
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 60 new}%
    \advance\pgfutil@tempdimb by -0.5\pgflinewidth%
  \fi
    \pgfarrowsleftextend{+-.5\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 60 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 60 new}%
    \advance\pgfutil@tempdima by -1.5\pgflinewidth% -(1+0.5)
    \pgftransformxshift{\pgfutil@tempdima}
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(30)}  
    \pgfpathmoveto{\pgfqpointpolar{150}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-150}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi    
}

% alternative open triangle 60 reversed
\pgfarrowsdeclare{open triangle 60 new reversed}{open triangle 60 new reversed}
{
  \ifdim\pgfgetarrowoptions{open triangle 60 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%   
    \pgfutil@tempdimb=7.794\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth% 
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 60 new reversed}%
    \advance\pgfutil@tempdimb by -\pgflinewidth%
  \fi
  \pgfarrowsleftextend{+-\pgflinewidth}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 60 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%  
    \pgfpathmoveto{\pgfqpointpolar{30}{9\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-30}{9\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 60 new reversed}%
    \advance\pgfutil@tempdima by -1.5\pgflinewidth% -(1+0.5)
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(30)}    
    \pgfpathmoveto{\pgfqpointpolar{30}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-30}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi  
}

% alternative open triangle 90 arrow
\pgfarrowsdeclare{open triangle 90 new}{open triangle 90 new}
{
  \ifdim\pgfgetarrowoptions{open triangle 90 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=6\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.707\pgflinewidth%
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 90 new}%
    \advance\pgfutil@tempdimb by -0.5\pgflinewidth%
  \fi
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 90 new}<0pt%  
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth% 
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{6\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 90 new}%
    \advance\pgfutil@tempdima by -1.20711\pgflinewidth% -(0.70711+0.5)  
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi    
}

% alternative open triangle 90 reversed arrow
\pgfarrowsdeclare{open triangle 90 new reversed}{open triangle 90 new reversed}
{
  \ifdim\pgfgetarrowoptions{open triangle 90 new reversed}<0pt%  
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfarrowsleftextend{+-.707\pgflinewidth}
    \pgfutil@tempdimb=6\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 90 new reversed}%
    \advance\pgfutil@tempdimb by -0.70711\pgflinewidth%
    \pgfarrowsleftextend{+-0.70711\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 90 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{6\pgfutil@tempdima}{6\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
   \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 90 new reversed}%
    \advance\pgfutil@tempdima by -1.20711\pgflinewidth% -(0.70711+0.5)   
    \pgfpathmoveto{\pgfqpoint{\pgfutil@tempdima}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpoint{\pgfutil@tempdima}{-\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi  
}

% alternative right hook arrow
\pgfarrowsdeclare{right hook new}{right hook new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \ifdim\pgfgetarrowoptions{right hook new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right hook new}%
    \pgfutil@tempdima=0.3125\pgfutil@tempdima%
    \advance\pgfutil@tempdima by 0.1875\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{right hook new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right hook new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 12%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{-1.665\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{-3\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.75\pgfutil@tempdima}{-4.665\pgfutil@tempdima}}
    {\pgfqpoint{2.415\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative right hook reversed arrow
\pgfarrowsdeclarereversed{right hook new reversed}{right hook new reversed}{right hook new}{right hook new}

% alternative right to arrow
\pgfarrowsdeclare{right to new}{right to new}
{
  \ifdim\pgfgetarrowoptions{right to new}<0pt%
    \pgfutil@tempdima=-0.84pt%
    \advance\pgfutil@tempdima by-1.3\pgflinewidth%
    \pgfutil@tempdimb=0.21pt%
    \advance\pgfutil@tempdimb by.625\pgflinewidth%
    \pgfarrowsleftextend{+\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% arbitrary value (2*0.5*0.8\pgflinewidth)
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.8\pgflinewidth}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{right to new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
    \pgfutil@tempdimb=0pt%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
    \pgfutil@tempdimb=0.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.4\pgflinewidth% arbitrary value (0.5*0.8\pgflinewidth)
    \pgftransformxshift{-\pgfutil@tempdimb}
  \fi  
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{-0.25\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
    {\pgfqpoint{0.55\pgfutil@tempdima}{0.125\pgflinewidth}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{0.125\pgflinewidth}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{0.125\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{\pgfutil@tempdimb}{0.125\pgflinewidth}}
  \pgfusepathqstroke
}

% alternative right to reversed arrow
\pgfarrowsdeclare{right to new reversed}{right to new reversed}
{
 \pgfarrowsleftextend{+-.1\pgflinewidth}
  \ifdim\pgfgetarrowoptions{right to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth% 
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.9\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right to new reversed}%
    \advance\pgfutil@tempdima by 0.1\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{right to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right to new reversed}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth 
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap 
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4\pgfutil@tempdima}}
    \pgfpathcurveto
      {\pgfqpoint{3.5\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
      {\pgfqpoint{0.75\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}
      {\pgfqpoint{0pt}{-0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4\pgfutil@tempdima}}
    \pgfpathcurveto
      {\pgfqpoint{3.5\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
      {\pgfqpoint{0.75\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}
      {\pgfqpoint{0pt}{0.125\pgflinewidth}}
  }
  \pgfusepathqstroke
}

% original round cap arrow (just for completeness)
\pgfarrowsdeclare{round cap new}{round cap new}
{
  \pgfarrowsleftextend{+0pt}
  \pgfarrowsrightextend{+\pgflinewidth}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}

% original serif cm arrow (just for completeness)
\pgfarrowsdeclare{serif cm new}{serif cm new}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.45\pgflinewidth%
  \pgfarrowsleftextend{+-.75\pgfutil@tempdima}
  \pgfarrowsrightextend{+.04\pgflinewidth}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.45\pgflinewidth%
  \pgftransformxshift{.04\pgflinewidth}
  \pgfpathmoveto{\pgfqpoint{-.75\pgfutil@tempdima}{.5\pgflinewidth}}
  \pgfpathcurveto
    {\pgfqpoint{-.375\pgfutil@tempdima}{.5\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{.7\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{1.95\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{1.95\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-.04\pgflinewidth}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-.04\pgflinewidth}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{-1.95\pgfutil@tempdima}}  
  \pgfpathlineto{\pgfqpoint{-.375\pgfutil@tempdima}{-1.95\pgfutil@tempdima}}  
  \pgfpathcurveto
    {\pgfqpoint{-.375\pgfutil@tempdima}{-.7\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{-.5\pgflinewidth}}
    {\pgfqpoint{-.75\pgfutil@tempdima}{-.5\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}

% original space arrow (just for completeness)
\pgfarrowsdeclare{space new}{space new}
{
  \pgfutil@tempdima=0.88pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{0pt}
  \pgfarrowsrightextend{\pgfutil@tempdima}
}
{}

% alternative square arrow
\pgfarrowsdeclare{square new}{square new}
{
  \ifdim\pgfgetarrowoptions{square new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \advance\pgfutil@tempdima by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{square new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsleftextend{+-.5\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{square new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{square new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 8%
    \pgftransformxshift{7\pgfutil@tempdima}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{1\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-7\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-7\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{1\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

% alternative stealth arrow
\pgfarrowsdeclare{stealth new}{stealth new}
{
  \ifdim\pgfgetarrowoptions{stealth new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \pgfutil@tempdimb=\pgflinewidth%
    \ifdim\pgfinnerlinewidth>0pt%
      \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
    \fi
    \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{stealth new}%
    \divide\pgfutil@tempdima by 8%
  \fi
  \pgfarrowsleftextend{+-3\pgfutil@tempdima}
  \pgfarrowsrightextend{+5\pgfutil@tempdima}
}
{
  \ifdim\pgfgetarrowoptions{stealth new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \pgfutil@tempdimb=\pgflinewidth%
    \ifdim\pgfinnerlinewidth>0pt%
      \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
    \fi
    \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{stealth new}%
    \divide\pgfutil@tempdima by 8%
  \fi
  \pgfpathmoveto{\pgfqpoint{5\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqfill
}

% alternative stealth reversed arrow
\pgfarrowsdeclarereversed{stealth new reversed}{stealth new reversed}{stealth new}{stealth new}

% alternative stealth' arrow
\pgfarrowsdeclare{stealth' new}{stealth' new}
{
  \ifdim\pgfgetarrowoptions{stealth' new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
    \pgfutil@tempdimb=6\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=2\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{stealth' new}%
    \pgfutil@tempdimb=0.71875\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.21875\pgflinewidth%
    \advance\pgfutil@tempdima by -\pgfutil@tempdimb%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \fi  
}
{
  \ifdim\pgfgetarrowoptions{stealth' new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{stealth' new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 8%
    \pgftransformxshift{3.75\pgfutil@tempdima}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-3\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
    {\pgfqpoint{-6\pgfutil@tempdima}{3.25\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-3\pgfutil@tempdima}{1\pgfutil@tempdima}}
    {\pgfqpoint{-3\pgfutil@tempdima}{-1\pgfutil@tempdima}}
    {\pgfqpoint{-6\pgfutil@tempdima}{-3.25\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-3\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
    {\pgfqpoint{-.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

% alternative stealth' reversed arrow
\pgfarrowsdeclarereversed{stealth' new reversed}{stealth' new reversed}{stealth' new}{stealth' new}

% alternative to arrow
\pgfarrowsdeclare{to new}{to new}
{
  \ifdim\pgfgetarrowoptions{to new}<0pt%
    \pgfutil@tempdima=-0.84pt%
    \advance\pgfutil@tempdima by-1.3\pgflinewidth%
    \pgfutil@tempdimb=0.21pt%
    \advance\pgfutil@tempdimb by.625\pgflinewidth%
    \pgfarrowsleftextend{+\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% arbitrary value (2*0.5*0.8\pgflinewidth)
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.8\pgflinewidth}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{to new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
    \pgfutil@tempdimb=0.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.4\pgflinewidth% arbitrary value (0.5*0.8\pgflinewidth)
    \pgftransformxshift{-\pgfutil@tempdimb}
  \fi
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{0.25\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
    {\pgfqpoint{0pt}{-0.25\pgfutil@tempdima}}
    {\pgfqpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
    {\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative to reversed arrow
\pgfarrowsdeclare{to new reversed}{to new reversed}
{
  \ifdim\pgfgetarrowoptions{to new reversed}<0pt%
    \pgfutil@tempdima=-0.21pt%
    \advance\pgfutil@tempdima by-0.475\pgflinewidth%
    \pgfutil@tempdimb=0.98pt%
    \advance\pgfutil@tempdimb by1.45\pgflinewidth%
    \pgfarrowsleftextend{+\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{to new reversed}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% arbitrary value (2*0.5*0.8\pgflinewidth)
    \pgfarrowsleftextend{+-0.8\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{to new reversed}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
    \pgfutil@tempdimb=0.25\pgfutil@tempdima%  
    \advance\pgfutil@tempdimb by -0.4\pgflinewidth% arbitrary value (0.5*0.8\pgflinewidth)
    \pgftransformxshift{\pgfutil@tempdimb}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfsetlinewidth{+0.8\pgflinewidth}
  \pgfpathmoveto{\pgfqpoint{3.5\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.25\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{0.25\pgfutil@tempdima}}
    {\pgfqpoint{-0.25\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{0.5\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}
    {\pgfqpoint{3.25\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
    {\pgfqpoint{3.5\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative triangle 45 arrow
\pgfarrowsdeclare{triangle 45 new}{triangle 45 new}
{
  \ifdim\pgfgetarrowoptions{triangle 45 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=8.705\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by1.28\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfarrowsleftextend{+-0.5\pgflinewidth}
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 45 new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%   
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{triangle 45 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                  {\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 45 new}%
    \advance\pgfutil@tempdima by -1.80656\pgflinewidth% -(1.30656+0.5)
    \pgftransformxshift{\pgfutil@tempdima}
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(22.5)}    
    \pgfpathmoveto{\pgfqpointpolar{157.5}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-157.5}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \fi
}

% alternative triangle 45 reversed arrow
\pgfarrowsdeclarereversed{triangle 45 new reversed}{triangle 45 new reversed}{triangle 45 new}{triangle 45 new}

% alternative triangle 60 arrow
\pgfarrowsdeclare{triangle 60 new}{triangle 60 new}
{
  \ifdim\pgfgetarrowoptions{triangle 60 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=7.29\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfarrowsleftextend{+-0.5\pgflinewidth}
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 60 new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%   
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{triangle 60 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%   
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 60 new}%
    \advance\pgfutil@tempdima by -1.5\pgflinewidth% -(1+0.5)
    \pgftransformxshift{\pgfutil@tempdima}
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(30)}    
    \pgfpathmoveto{\pgfqpointpolar{150}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-150}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \fi
}

% alternative triangle 60 reversed arrow
\pgfarrowsdeclarereversed{triangle 60 new reversed}{triangle 60 new reversed}{triangle 60 new}{triangle 60 new}

% alternative triangle 90 arrow
\pgfarrowsdeclare{triangle 90 new}{triangle 90 new}
{
  \ifdim\pgfgetarrowoptions{triangle 90 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=5.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.707\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfarrowsleftextend{+-0.5\pgflinewidth}
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 90 new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{triangle 90 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfqpoint{-5.5\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{-5.5\pgfutil@tempdima}{6\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 90 new}%
    \advance\pgfutil@tempdima by -1.20711\pgflinewidth% -(0.70711+0.5)
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \fi
}

% alternative triangle 90 reversed arrow
\pgfarrowsdeclarereversed{triangle 90 new reversed}{triangle 90 new reversed}{triangle 90 new}{triangle 90 new}

% original triangle 90 cap arrow (just for completeness)
\pgfarrowsdeclare{triangle 90 cap new}{triangle 90 cap new}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+\pgflinewidth}
}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfusepathqfill
}

% original triangle 90 cap reversed arrow (just for completeness)
\pgfarrowsdeclare{triangle 90 cap new reversed}{triangle 90 cap new reversed}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+\pgflinewidth}
}
{
  \pgfpathmoveto{\pgfqpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0\pgflinewidth}}
  \pgfusepathqfill
}

% alias alternative to arrow
\pgfarrowsdeclarealias{< new}{> new}{to new}{to new}

% alias alternative to reversed arrow
\pgfarrowsdeclarealias{> new}{< new}{to new reversed}{to new reversed}

% arrow head length code
\pgfsetarrowoptions{* new}{-1pt}
\pgfsetarrowoptions{< new}{-1pt}
\pgfsetarrowoptions{> new}{-1pt}
\pgfsetarrowoptions{) new}{-1pt}
\pgfsetarrowoptions{( new}{-1pt}
\pgfsetarrowoptions{[ new}{-1pt}
\pgfsetarrowoptions{] new}{-1pt}
\pgfsetarrowoptions{| new}{-1pt}
\pgfsetarrowoptions{angle 45 new}{-1pt}
\pgfsetarrowoptions{angle 45 new reversed}{-1pt}
\pgfsetarrowoptions{angle 60 new}{-1pt}
\pgfsetarrowoptions{angle 60 new reversed}{-1pt}
\pgfsetarrowoptions{angle 90 new}{-1pt}
\pgfsetarrowoptions{angle 90 new reversed}{-1pt}
\pgfsetarrowoptions{diamond new}{-1pt}
\pgfsetarrowoptions{hooks new}{-1pt}
\pgfsetarrowoptions{hooks new reversed}{-1pt}
\pgfsetarrowoptions{latex new}{-1pt}
\pgfsetarrowoptions{latex new reversed}{-1pt}
\pgfsetarrowoptions{latex' new}{-1pt}
\pgfsetarrowoptions{latex' new reversed}{-1pt}
\pgfsetarrowoptions{left hook new}{-1pt}
\pgfsetarrowoptions{left hook new reversed}{-1pt}
\pgfsetarrowoptions{left to new}{-1pt}
\pgfsetarrowoptions{left to new reversed}{-1pt}
\pgfsetarrowoptions{o new}{-1pt}
\pgfsetarrowoptions{open diamond new}{-1pt}
\pgfsetarrowoptions{open square new}{-1pt}
\pgfsetarrowoptions{open triangle 45 new}{-1pt}
\pgfsetarrowoptions{open triangle 45 new reversed}{-1pt}
\pgfsetarrowoptions{open triangle 60 new}{-1pt}
\pgfsetarrowoptions{open triangle 60 new reversed}{-1pt}
\pgfsetarrowoptions{open triangle 90 new}{-1pt}
\pgfsetarrowoptions{open triangle 90 new reversed}{-1pt}
\pgfsetarrowoptions{right hook new}{-1pt}
\pgfsetarrowoptions{right hook new reversed}{-1pt}
\pgfsetarrowoptions{right to new}{-1pt}
\pgfsetarrowoptions{right to new reversed}{-1pt}
\pgfsetarrowoptions{square new}{-1pt}
\pgfsetarrowoptions{stealth new}{-1pt}
\pgfsetarrowoptions{stealth new reversed}{-1pt}
\pgfsetarrowoptions{stealth' new}{-1pt}
\pgfsetarrowoptions{stealth' new reversed}{-1pt}
\pgfsetarrowoptions{to new}{-1pt}
\pgfsetarrowoptions{to new reversed}{-1pt}
\pgfsetarrowoptions{triangle 45 new}{-1pt}
\pgfsetarrowoptions{triangle 45 new reversed}{-1pt}
\pgfsetarrowoptions{triangle 60 new}{-1pt}
\pgfsetarrowoptions{triangle 60 new reversed}{-1pt}
\pgfsetarrowoptions{triangle 90 new}{-1pt}
\pgfsetarrowoptions{triangle 90 new reversed}{-1pt}

\pgfkeys{/tikz/.cd, arrow head/.default=-1pt, arrow head/.code={%
  \pgfsetarrowoptions{* new}{#1}%
  \pgfsetarrowoptions{< new}{#1}%
  \pgfsetarrowoptions{> new}{#1}%
  \pgfsetarrowoptions{) new}{#1}%
  \pgfsetarrowoptions{( new}{#1}%
  \pgfsetarrowoptions{[ new}{#1}%
  \pgfsetarrowoptions{] new}{#1}%
  \pgfsetarrowoptions{| new}{#1}%
  \pgfsetarrowoptions{angle 45 new}{#1}%
  \pgfsetarrowoptions{angle 45 new reversed}{#1}%
  \pgfsetarrowoptions{angle 60 new}{#1}%
  \pgfsetarrowoptions{angle 60 new reversed}{#1}%
  \pgfsetarrowoptions{angle 90 new}{#1}%
  \pgfsetarrowoptions{angle 90 new reversed}{#1}%
  \pgfsetarrowoptions{diamond new}{#1}%
  \pgfsetarrowoptions{hooks new}{#1}%
  \pgfsetarrowoptions{hooks new reversed}{#1}%
  \pgfsetarrowoptions{latex new}{#1}%
  \pgfsetarrowoptions{latex new reversed}{#1}%
  \pgfsetarrowoptions{latex' new}{#1}%
  \pgfsetarrowoptions{latex' new reversed}{#1}%
  \pgfsetarrowoptions{left hook new}{#1}%
  \pgfsetarrowoptions{left hook new reversed}{#1}%
  \pgfsetarrowoptions{left to new}{#1}%
  \pgfsetarrowoptions{left to new reversed}{#1}%
  \pgfsetarrowoptions{o new}{#1}%
  \pgfsetarrowoptions{open diamond new}{#1}%
  \pgfsetarrowoptions{open square new}{#1}%
  \pgfsetarrowoptions{open triangle 45 new}{#1}%
  \pgfsetarrowoptions{open triangle 45 new reversed}{#1}%
  \pgfsetarrowoptions{open triangle 60 new}{#1}%
  \pgfsetarrowoptions{open triangle 60 new reversed}{#1}%
  \pgfsetarrowoptions{open triangle 90 new}{#1}%
  \pgfsetarrowoptions{open triangle 90 new reversed}{#1}%
  \pgfsetarrowoptions{right hook new}{#1}%
  \pgfsetarrowoptions{right hook new reversed}{#1}%
  \pgfsetarrowoptions{right to new}{#1}%
  \pgfsetarrowoptions{right to new reversed}{#1}%
  \pgfsetarrowoptions{square new}{#1}%
  \pgfsetarrowoptions{stealth new}{#1}%
  \pgfsetarrowoptions{stealth new reversed}{#1}%
  \pgfsetarrowoptions{stealth' new}{#1}%
  \pgfsetarrowoptions{stealth' new reversed}{#1}%
  \pgfsetarrowoptions{to new}{#1}%
  \pgfsetarrowoptions{to new reversed}{#1}%
  \pgfsetarrowoptions{triangle 45 new}{#1}%
  \pgfsetarrowoptions{triangle 45 new reversed}{#1}%
  \pgfsetarrowoptions{triangle 60 new}{#1}%
  \pgfsetarrowoptions{triangle 60 new reversed}{#1}%
  \pgfsetarrowoptions{triangle 90 new}{#1}%
  \pgfsetarrowoptions{triangle 90 new reversed}{#1}%
}}

\endinput

==> preamble-common.tex <==
\newcommand{\blurb}[1]{}

%\newenvironment{enumerateroman}{\begin{enumerate}[(i)]}{\end{enumerate}}
\newcommand{\axref}[1]{\ref{#1}}
\newcommand{\preaxref}[1]{\ref{#1}}
\newcommand{\axrefrange}[2]{\ref{#1}--\ref{#2}}
\newcommand{\preaxrefrange}[2]{\ref{#1}--\ref{#2}}
\newlist{myaxioms}{enumerate}{10}
\setlist[myaxioms,1]{label=(P\arabic*)}
\setlist[myaxioms]{resume}
\newenvironment{axioms}{\begin{myaxioms}[resume*=myaxiomsseries]}{\end{myaxioms}}
    % {\usecounter{axiomcounter}
    % \setlength{\rightmargin}{\leftmargin}}}{\end{list}}
\newlist{enumeratei}{enumerate}{10}
\setlist[enumeratei]{label=\emph{(\roman*)}}

\usepackage{tikz,tikz-cats}
\tikzset{todim/.style = {decoration={markings, mark=at position .5 with %
      {\draw (-1pt,-1pt) rectangle (1pt,1pt);}},postaction={decorate}}}
\renewcommand{\diaggrandhauteur}{.6}
\renewcommand{\diaggrandlargeur}{1.3}


%\pagestyle{plain}

\hyphenation{co-mo-noid hir-scho-witz}
% operators
\DeclareMathOperator{\ob}{ob}
\DeclareMathOperator{\mor}{mor}
\DeclareMathOperator{\Dim}{dim}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\lift}{lift}
\DeclareMathOperator{\cod}{cod}
\DeclareMathOperator{\domv}{dom_{\mathit{v}}}
\DeclareMathOperator{\codv}{cod_{\mathit{v}}}
\DeclareMathOperator{\domh}{dom_{\mathit{h}}}
\DeclareMathOperator{\codh}{cod_{\mathit{h}}}
\DeclareMathOperator{\Dom}{Dom}
\DeclareMathOperator{\Cod}{Cod}
\DeclareMathOperator{\Sub}{Sub}
\DeclareMathOperator{\el}{el}
\DeclareMathOperator{\lan}{lan}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\ccolim}{\bigcat{colim}}
\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\Fam}{Fam}
\DeclareMathOperator{\Leaves}{Leaves}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\injl}{inj_l}
\DeclareMathOperator{\injr}{inj_r}
\newcommand{\cob}[1]{\Delta_{#1}}
\newcommand{\cocob}[1]{\Sigma_{#1}}
\newcommand{\compo}[1]{\lsem #1 \rsem}
\newcommand{\compofun}{\compo{-}}
\newcommand{\comp}{\bigcat{comp}}
\newcommand{\restr}[2]{#1_{|#2}}
\newcommand{\Restr}[2]{#1_{||#2}}
\newcommand{\two}{\mathsf{2}}
\newcommand{\liftings}[2]{#1 {\uparrow} #2}
\renewcommand{\emptyset}{\varnothing}

% formating 
\newcommand{\intro}[1]{\emph{#1}}
\newcommand{\bigcat}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\maji}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\bigfun}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\cat}[1]{\mathbf{#1}}
\newcommand{\fonc}[1]{\mathsf{#1}}
\newcommand{\dbr}[1]{\left \lsem {#1} \right \rsem}
\newcommand{\cd}[2][]{\vcenter{\hbox{\xymatrix#1{#2}}}}
\newcommand{\Formulae}{\maji{F}}
\newcommand{\Vars}{\bigcat{Vars}}
\newcommand{\TVars}{\bigcat{TVars}}
\newcommand{\Names}{\bigcat{Names}}
\newcommand{\Sequents}{\mathit{Sq}}
\newcommand{\commentthis}[1]{}
\newcommand{\pow}{\mathcal{P}}
\newcommand{\powfin}{\mathcal{P}_f}
\newcommand{\Psh}[1]{\widehat{#1}}
\newcommand{\CVvtoCATfun}{\SS^v_{-}}
\newcommand{\CVvtoCAT}[1]{\SS^v_{#1}}
\newcommand{\CEvtoCATfun}{\SS^V_{-}}
\newcommand{\CEvtoCAT}[1]{\SS^V_{#1}}
\renewcommand{\P}{\maji{P}}
\newcommand{\Phat}{\widehat{\P}}
\newcommand{\ruleref}[1]{\textsc{#1}}
\newcommand{\Cospan}[1]{\bigcat{Cospan} (#1)}
\newcommand{\Span}[1]{\bigcat{Span} (#1)}
\newcommand{\Cospanf}[1]{\bigcat{Cospan}_f (#1)}
\newcommand{\into}{\hookrightarrow}
\newcommand{\otni}{\hookleftarrow}
\newcommand{\onto}{\twoheadrightarrow}
\newcommand{\otno}{\twoheadleftarrow}
\newcommand{\ot}{\leftarrow}
\newcommand{\xto}[1]{\xrightarrow{#1}}
\newcommand{\xot}[1]{\xleftarrow{#1}}
\newcommand{\xotstar}[1]{\mathrel{\xleftarrow{#1}^\star}}
\newcommand{\xtostar}[1]{\mathrel{\xrightarrow{#1}^\star}}
\newcommand{\tostar}{\mathrel{\to^\star}}
\newcommand{\xTo}[1]{\xRightarrow{#1}}
\newcommand{\xOt}[1]{\xLeftarrow{#1}}
\newcommand{\xOtstar}[1]{\mathrel{\xLeftarrow{#1}^\star}}
\newcommand{\xTrans}[2]{\mathrel{{}_{#1}\!\xOt{#2}}}
\newcommand{\xtrans}[2]{\mathrel{{}_{#1}\!\xot{#2}}}
\newcommand{\xinto}[1]{\xarrow[into]{#1}}
\newcommand{\xotni}[1]{\xarrow[linto]{#1}}
% \newcommand{\shortrightarrow}{%
%   \mathrel{\tikz [->,baseline=-.75ex] \draw (0,0) -- (.6em,0) ;}}
% \newcommand{\shortleftarrow}{%
%   \mathrel{\tikz [<-,baseline=-.75ex] \draw (0,0) -- (.6em,0) ;}}
% \newcommand{\rightarrowtriangle}{%
%   \mathrel{\tikz [-open triangle 45,baseline=-.75ex] \draw (0,0) -- (.6em,0) ;}}
% \newcommand{\xinto}[1]{\xhookrightarrow{#1}}
% \newcommand{\xotni}[1]{\xhookleftarrow{#1}}
%\newcommand{\xonto}[1]{\xtwoheadtrightarrow{#1}}
%\newcommand{\xotno}[1]{\xtwoheadleftarrow{#1}}
\newcommand{\pto}{\rightharpoonup}
\newcommand{\todim}{\rightarrowtriangle}
\newcommand{\compat}{\mathbin{\triangleright}}
\newcommand{\compatible}[3]{(#1,#2) \triangleright #3}
\newcommand{\compatSierp}{\compat^\Sierp}
\newcommand{\compatibleSierp}[3]{(#1,#2) \compatSierp #3}
\newcommand{\compatL}{\compat^{\LLL}}
\newcommand{\compatibleL}[3]{(#1,#2) \compatL #3}
\newcommand{\Lcompat}{\LLL^{\compat}}
\newcommand{\LiW}{\LLL^{\id/\W}}

\newcommand{\compatof}[1]{\compat^{#1}}
\newcommand{\compatibleof}[4]{(#2,#3) \compatof{#1} #4}
\newcommand{\ofcompat}[1]{#1^{\compat}}

\newcommand{\compatastar}{\compatof{A^\star}}
\newcommand{\compatfca}{\compatof{\freecat{A}}}
\newcommand{\freecat}[1]{\freecatfun(#1)}
\newcommand{\freecatfun}{\mathsf{fc}}


\newcommand{\LG}[1]{\mathrm{LG}/#1}

\newcommand{\botG}{\bot^{G}}
\newcommand{\botGa}{\bot^G_A}
\newcommand{\botHa}{\bot^H_A}
\newcommand{\botGb}{\bot^G_B}

\newcommand{\labelof}[1]{\ell^{#1}}
\newcommand{\labelQFI}{\labelof{\QFI}}
\newcommand{\labelpi}{\labelof{\picalc}}

\newcommand{\labelSSSI}{\labelof{{\SSSI}}}
\newcommand{\labelSSS}{\labelof{{\SSS}}}
\newcommand{\labelLLL}{\labelof{{\LLL}}}

\newcommand{\labelC}{\ell^\C}
\newcommand{\compatC}{\compat^\C}
\newcommand{\compatibleC}[3]{(#1,#2) \compatC #3}
\newcommand{\CW}{\C^{\W}}
\newcommand{\Ccoh}{\C^{\coh}}


\newcommand{\labelG}{\ell^G}
\newcommand{\labelfcG}{\ell^{\freecat{G}}}
\newcommand{\compatG}{\compat^G}
\newcommand{\compatGstar}{\compatof{G^\star}}
\newcommand{\compatfcG}{\compatof{\freecat{G}}}
\newcommand{\compatibleG}[3]{(#1,#2) \compatG #3}
\newcommand{\Gcompat}{G^{\compat}}
\newcommand{\GW}{G^{\W}}
\newcommand{\Gcoh}{G^{\coh}}
\newcommand{\Ga}{{G{\compat}A}}
\newcommand{\Gb}{{G{\compat}B}}
\newcommand{\labelGi}{\ell^{G'}}
\newcommand{\compatGi}{\compat^{G'}}
\newcommand{\compatibleGi}[3]{(#1,#2) \compatGi #3}
\newcommand{\Gicompat}{{Gi}^{\compat}}
\newcommand{\Atrees}{\HHH}
\newcommand{\fG}{f^*(G)}
\newcommand{\fGa}{{\fG{\compat}A}}

\newcommand{\labelH}{\ell^H}
\newcommand{\compatH}{\compat^H}
\newcommand{\compatibleH}[3]{(#1,#2) \compatH #3}
\newcommand{\Hcompat}{H^{\compat}}
\newcommand{\HW}{H^{\W}}

\newcommand{\dpara}{\Downarrow}

\newcommand{\labelA}{\ell^\A}
\newcommand{\compatA}{\compat^\A}
\newcommand{\compatibleA}[3]{#1 \parallel #2 = #3} %{(#1,#2) \compatA #3}
\newcommand{\Acompat}{\A^{\compat}}

\newcommand{\atrees}{\HHH^A}
\newcommand{\labela}{\ell^A}
\newcommand{\compata}{\compat^A}
\newcommand{\compatiblea}[3]{#1 \parallel #2 = #3} %{(#1,#2) \compata #3}
\newcommand{\acompat}{A^{\compat}}
\newcommand{\aW}{A^\W}
\newcommand{\acoh}{A^\coh}
%\newcommand{\faireqa}{\mathrel{\sim_{A}}}
%\newcommand{\fairneqa}{\mathrel{\nsim_{A}}}
\newcommand{\faireqof}[1]{\mathrel{\sim^{#1}_{f}}}
\newcommand{\faireqI}{\faireqof{\SSSI}}
\newcommand{\fairneqof}[1]{\mathrel{\nsim^{#1}_{f}}}
\newcommand{\faireqG}{\mathrel{\faireqof{G}}}
\newcommand{\fairneqG}{\mathrel{\fairneqof{G}}}
\newcommand{\faireqH}{\mathrel{\faireqof{H}}}
\newcommand{\botrela}{\mathrel{\bot_A}}
\newcommand{\nbotrela}{\mathrel{\notbot_A}}

%% A-tree equivalence
\newcommand{\treeqof}[2]{\mathrel{\sim^{#1|#2}_f}}
\newcommand{\treneqof}[2]{\mathrel{\nsim^{#1|#2}_f}}
\newcommand{\treeqGa}{\treeqof{G}{A}}
\newcommand{\faireqGa}{\mathrel{\treeqof{G}{A}}}
\newcommand{\faireqGb}{\mathrel{\treeqof{G}{B}}}
\newcommand{\fairneqGa}{\mathrel{\treneqof{G}{A}}}
\newcommand{\faireqHa}{\mathrel{\treeqof{H}{A}}}
\newcommand{\fairneqHa}{\mathrel{\treneqof{H}{A}}}
\newcommand{\botrelGa}{\mathrel{\bot^{G|A}}}
\newcommand{\nbotrelGa}{\mathrel{\notbot^{G|A}}}

\newcommand{\combineof}[1]{\mathbin{\diamond_{#1}}}
\newcommand{\combine}[3]{#2 \combineof{#1} #3}
\newcommand{\combinea}[2]{\combine{A}{#1}{#2}}
\newcommand{\combineA}[2]{\combine{\A}{#1}{#2}}

\newcommand{\labelb}{\ell^B}
\newcommand{\compatb}{\compat^B}
\newcommand{\compatibleb}[3]{(#1,#2) \compatb #3}
\newcommand{\bcompat}{B^{\compat}}
\newcommand{\bW}{B^\W}
\newcommand{\bcoh}{B^\coh}

\newcommand{\pW}{p^\W}
\newcommand{\pcoh}{p^\coh}

\newcommand{\fW}{f^\W}
\newcommand{\fcoh}{f^\coh}

\newcommand{\fcompat}{f^{\compat}}


% text
\newcommand{\ie}{i.e.,}
\newcommand{\eg}{e.g.,}

% Variables
\renewcommand{\hat}[1]{\widehat{#1}}
\newcommand{\bsig}{\maji{K}} % binding signature
\newcommand{\model}{\maji{L}} % a \Sigma_\bsig model
\newcommand{\bbig}{M} % category of binding bigraphs
\newcommand{\theory}{\maji{T}}
\newcommand{\sig}{\Sigma}



%\numberwithin{equation}{section} 
%\numberwithin{paragraph}{section}


\DeclareMathOperator{\Ran}{Ran}\DeclareMathOperator{\Lan}{Lan} \DeclareMathOperator{\Und}{Und}
\DeclareMathOperator{\Inc}{Inc} \DeclareMathOperator{\Alg}{-Alg} 
\DeclareMathOperator{\Mnd}{Mnd}
\DeclareMathOperator{\Law}{Law}
\DeclareMathOperator{\etant}{\eta_{\nt}}
\DeclareMathOperator{\etacolon}{\eta_{:}}


\def\framed{%
\setbox0=\vbox\bgroup%
\advance\hsize by -2\fboxsep\advance\hsize by -2\fboxrule%
\linewidth=\hsize%
}
\def\endframed{%
\egroup\noindent\framebox[\textwidth]{\box0}\vspace*{1mm}}



\usepackage{color}
\definecolor{dkgreen}{rgb}{0,0.2,0}
\newcommand{\todo}[1]{\marginpar{\textcolor{dkgreen}{#1}}}


\newcommand{\A}{\maji{A}}
\newcommand{\Abar}{\overline{\maji{A}}}
\newcommand{\AW}{\A^{\W}}
\newcommand{\Acoh}{\A^\coh}
\renewcommand{\AA}{\bigcat{A}}
\newcommand{\AAA}{\bigfun{A}}
\newcommand{\APi}{P1}
\newcommand{\APii}{P2}
\newcommand{\APiii}{P3}
\newcommand{\APiv}{P4}
\newcommand{\APv}{P5}
\newcommand{\APvi}{P6}
\newcommand{\B}{\maji{B}}
\newcommand{\Beh}[1]{\Behfun_{#1}}
\newcommand{\Behfun}{\bigcat{B}}
\newcommand{\NaiveStrats}[1]{\bigcat{S}_{#1}}
\newcommand{\LocalStrats}{\bigcat{B}}
\newcommand{\BB}{\bigcat{B}}
\newcommand{\BsofF}{\chi}
\newcommand{\BofF}{\ulcorner \chi \urcorner}
\newcommand{\BiVi}{\bigcat{V}}
\newcommand{\C}{\maji{C}}
\newcommand{\CC}{\bigcat{C}}
\newcommand{\CMM}{\bigcat{CM}}
\newcommand{\CCC}{\bigfun{C}}
\newcommand{\Ci}{\maji{C}_1}
\newcommand{\Cii}{\maji{C}_2}
\newcommand{\Ctau}{\maji{C}_\tau}
\newcommand{\Cio}{\C_{\iota/o}}
\newcommand{\Cpara}{\maji{C}_{\para}}
\newcommand{\Cparan}{\maji{C}_{\para_n}}
\newcommand{\Cparam}{\maji{C}_{\para_m}}
\newcommand{\Cnu}{\maji{C}_{\nu}}
\newcommand{\Cnun}{\maji{C}_{\nu_n}}
\newcommand{\Cnum}{\maji{C}_{\nu_m}}
\newcommand{\tick}{\daimon}
\newcommand{\closedtick}{\xi}
\newcommand{\Ctick}{\maji{C}_{\tick}}
\newcommand{\Ctickn}{\maji{C}_{\tick_n}}
\newcommand{\Ctickm}{\maji{C}_{\tick_m}}
\newcommand{\Cni}{\C_{n,i}}
\newcommand{\Cnimj}{\C_{n,i,m,j}}
\newcommand{\Cnimjprime}{\C_{n',i',m',j'}}
\newcommand{\Cn}{[n]}
\newcommand{\Csn}{[n + 1]}
\newcommand{\Cm}{[m]}
\newcommand{\Csm}{[m+1]}
\newcommand{\Cg}{[g]}
\newcommand{\Chat}{\hat{\maji{C}}}
\newcommand{\Chatf}{\Pshf{\maji{C}}}
\newcommand{\Chatc}{\Pshc{\maji{C}}}
\newcommand{\Chato}{\OPsh{\maji{C}}}
\newcommand{\Cihat}{\hat{\maji{\C}_1}}
\newcommand{\Ciihat}{\hat{\maji{\C}_2}}
\newcommand{\Ctauhat}{\hat{\maji{\C}_\tau}}
\newcommand{\Cnuhat}{\hat{\maji{\C}_\nu}}
\newcommand{\Cpos}[1]{\C^+_{#1}}
\newcommand{\Cneg}[1]{\C^-_{#1}}
\newcommand{\Cposni}{\Cpos{n,i}}
\newcommand{\Cposmj}{\Cpos{m,j}}
\newcommand{\Cnegni}{\Cneg{n,i}}
\newcommand{\Cnegmj}{\Cneg{m,j}}
\newcommand{\CE}{\E}
\newcommand{\CEplus}{\E^+}
\newcommand{\CV}{\V}
\newcommand{\CEhat}{\widehat{\CE}}
\newcommand{\CEx}{\CE_x}
\newcommand{\CEn}{\CE_n}
\newcommand{\CVx}{\CV_x}
\newcommand{\CVX}{\CV_X}
\newcommand{\CVY}{\CV_Y}
\newcommand{\CVn}{\CV_{[n]}}
\newcommand{\CVm}{\CV_{[m]}}
\newcommand{\CVni}{\CV_{[n']}}
\newcommand{\CExhat}{\widehat{\CE_x}}
\newcommand{\CEXhat}{\widehat{\CE_X}}
\newcommand{\CEnhat}{\widehat{\CE_{[n]}}}
\newcommand{\CVxhat}{\widehat{\CV_x}}
\newcommand{\CVnhat}{\widehat{\CV_{[n]}}}
\newcommand{\CVnihat}{\widehat{\CV_{[n']}}}
\newcommand{\CVXhat}{\widehat{\CVX}}
\newcommand{\CVhat}{\widehat{\CV}}
\newcommand{\CVYhat}{\widehat{\CVY}}
\newcommand{\CVnhatf}{\OPsh{\CVn}}
\newcommand{\CVXhatf}{\OPsh{\CVX}}
\newcommand{\CVhatf}{\OPsh{\CV_{[-]}}}
\newcommand{\CEU}{\CE_U}
\newcommand{\CEX}{\CE_X}
\newcommand{\CEY}{\CE_Y}
\newcommand{\D}{\maji{D}}
\newcommand{\DD}{\bigcat{D}}
\newcommand{\Dseq}{\D_{\mathrm{seq}}}
\newcommand{\Dhat}{\widehat{\maji{D}}}
\renewcommand{\DH}{\D_{H}}
\newcommand{\DseqH}{(\Dseq)_{H}}
\newcommand{\Dh}{\D_h}
\newcommand{\Dtwo}{\D_{\langle 2 \rangle}}
\newcommand{\Dseqh}{(\Dseq)_h}
\newcommand{\Dv}{\D_v}
\newcommand{\Do}{\maji{D}^0}
\newcommand{\DoH}{\Do_{H}}
\newcommand{\Doh}{\Do_h}
\newcommand{\Dov}{\Do_v}
\newcommand{\ccs}{\mathit{CCS}}
\newcommand{\picalc}{\mathit{Pi}}
\newcommand{\Dccs}{\maji{D}^{\scriptscriptstyle \ccs}}
\newcommand{\DccsH}{\Dccs_{H}}
\newcommand{\Dccsh}{\Dccs_h}
\newcommand{\Dccsv}{\Dccs_v}
\newcommand{\Dccso}{\maji{D}^{\mathit{CCS},0}}
\newcommand{\DccsoH}{\Dccso_{H}}
\newcommand{\Dccsoh}{\Dccso_h}
\newcommand{\Dccsov}{\Dccso_v}
\newcommand{\Di}{\maji{D}^1}
\newcommand{\DiH}{\Di_{H}}
\newcommand{\Dih}{\Di_h}
\newcommand{\Div}{\Di_v}
\newcommand{\DV}{\D_V}
\newcommand{\DVi}{\V}
\newcommand{\DI}{\I}
\newcommand{\DA}{\A}
\newcommand{\DM}{\M}
\newcommand{\DB}{\B}
\newcommand{\DF}{\F}
\newcommand{\QF}{\Q}
\newcommand{\QFI}{\Q^I}
\newcommand{\QFS}{\Q^S}
\newcommand{\DFv}{\Dv^\F}
\newcommand{\DFB}{\F^1}
\newcommand{\DW}{\D^\W}
\newcommand{\DccsW}{(\Dccs)^\W}
\newcommand{\DE}{\E}
\newcommand{\E}{\maji{E}}
\newcommand{\EH}{\E_{H}}
\newcommand{\EV}{\E_V}
\newcommand{\Eh}{\B}
\newcommand{\Ev}{\E_v}
\newcommand{\Ehsq}{\E_{h,\Nat}}
\newcommand{\Ehsqiso}{\E^{\iso}_{h, \Nat}}
\newcommand{\EE}{\bigcat{E}}
\newcommand{\EC}{\EH^c}
\newcommand{\EVi}{\E^{\V}}
\newcommand{\EVihato}[1]{\OPsh{\E^{\V}_{#1}}}
\newcommand{\EVihatofun}{\EVihato{-}}
\newcommand{\EF}{\E^{\F}}
\newcommand{\EW}{\E^{\W}}
\newcommand{\F}{\maji{F}}
\newcommand{\FFF}{\bigfun{F}}
\newcommand{\FF}{\bigcat{F}}
\newcommand{\Fo}{\maji{F}_0}
\newcommand{\Fi}{\maji{F}_1}
\newcommand{\Fii}{\maji{F}_2}
\newcommand{\G}{\maji{G}}
\newcommand{\GG}{\bigcat{G}}
\newcommand{\GGG}{\bigfun{G}}
\newcommand{\GGX}{\GG_X}
\newcommand{\Gi}{\maji{G}_1}
\newcommand{\Gii}{\maji{G}_2}
\renewcommand{\H}{\maji{H}}
\newcommand{\HH}{\bigcat{H}}
\newcommand{\HHH}{\bigfun{H}}
\newcommand{\Ho}{\maji{H}_0}
\newcommand{\Hi}{\maji{H}_1}
\newcommand{\Hii}{\maji{H}_2}
\newcommand{\I}{\maji{I}}
\newcommand{\II}{\bigcat{I}}
\newcommand{\III}{\bigfun{I}}
\newcommand{\ii}{\bigcat{i}}
\newcommand{\iV}{\bigcat{i}_\DVi}
\newcommand{\xiiV}{\xi_{\iV}}
\newcommand{\iB}{\bigcat{i}_\DB}
\newcommand{\xiiB}{\xi_{\iB}}
\newcommand{\J}{\maji{J}}
\newcommand{\JJ}{\bigcat{J}}
\newcommand{\K}{\maji{K}}
\newcommand{\Ki}{\maji{K}_1}
\newcommand{\Kii}{\maji{K}_2}
\newcommand{\KKK}{\bigfun{K}}
\renewcommand{\L}{\maji{L}}
\newcommand{\LL}{\bigcat{L}}
\newcommand{\LLL}{\bigfun{L}}
\newcommand{\LLLcc}{\LLL_{\bigcat{cc}}}
\newcommand{\LLLlocal}{\bigfun{L}_{\mathrm{local}}}
\newcommand{\LLLind}{\bigfun{L}_{\mathrm{ind}}}
\newcommand{\LLLbar}{\overline{\bigfun{L}}}
\newcommand{\LLLW}{\LLL^\W}
\newcommand{\LLLlocalW}{\LLLlocal^\W}
\newcommand{\M}{\maji{M}}
\newcommand{\MM}{\bigcat{M}}
\newcommand{\MMM}{\bigfun{M}}
\newcommand{\griso}[1]{[#1]}
\newcommand{\MMMB}{\griso{\B}}
\newcommand{\MMMF}{\griso{\F}}
\newcommand{\MMMFr}{\griso{\F_\iota}}
\newcommand{\MMMFB}{\griso{\F^1}}
\newcommand{\MMMFplus}{\griso{\F^{+}}}
\newcommand{\MU}{\M_U}
\newcommand{\N}{\maji{N}}
\newcommand{\NN}{\bigcat{N}}
\newcommand{\NNN}{\bigfun{N}}
\newcommand{\U}{\maji{U}}
\newcommand{\UU}{\bigcat{U}}
\newcommand{\UUU}{\bigfun{U}}
\newcommand{\Uo}{\maji{U}_0}
\newcommand{\Ui}{\maji{U}_1}
\newcommand{\Uii}{\maji{U}_2}
\newcommand{\V}{\maji{V}}
\newcommand{\VH}{\V_H}
\newcommand{\VV}{\bigcat{V}}
\newcommand{\VVV}{\bigfun{V}}
\newcommand{\Vv}{\V_v}
\newcommand{\VViso}{\V^{\iso}_V}
\newcommand{\Vh}{\V_h}
\newcommand{\VX}{\V_X}
\newcommand{\Vx}{\V_x}
\newcommand{\VY}{\V_Y}
\newcommand{\Vo}{\maji{V}_0}
\newcommand{\Vi}{\maji{V}_1}
\newcommand{\Vii}{\maji{V}_2}
\newcommand{\W}{\maji{W}}
\newcommand{\Wccs}{\W_{\ccs}}
\newcommand{\ccsW}{\W_{\ccs}}
\newcommand{\WW}{\bigcat{W}}
\newcommand{\WWW}{\bigfun{W}}
\newcommand{\WWWcc}{\WWW_{\bigcat{cc}}}
\newcommand{\yoneda}{\bigcat{y}}
\newcommand{\CWEh}{\W_{\Eh}}
\newcommand{\CWEhhat}{\widehat{\WEh}}
\newcommand{\CWU}{\W_U}
\newcommand{\CWX}{\W_X}
\newcommand{\CWofX}{\W(X)}
\newcommand{\CWXhat}{\widehat{\WX}}
\newcommand{\CWhat}{\widehat{\W}}
\newcommand{\CWofXhat}{\widehat{\WofX}}
\newcommand{\CWY}{\W_Y}
\newcommand{\Wi}{\W_1}
\newcommand{\X}{\maji{X}}
\newcommand{\XX}{\bigcat{X}}
%\newcommand{\P}{\maji{P}}
\newcommand{\PP}{\bigcat{P}}
\newcommand{\PPP}{\bigfun{P}}
\newcommand{\PolyEnd}{\bigcat{PolyEnd}}
\newcommand{\Occ}{\maji{O}}
\newcommand{\PreOcc}{\maji{PreO}}
\newcommand{\occs}{\bigcat{occ}}
\newcommand{\access}{\bigcat{access}}
\newcommand{\biases}{\bigcat{B}}
\newcommand{\Q}{\maji{Q}}
\newcommand{\QQ}{\bigcat{Q}}
\newcommand{\R}{\maji{R}}
\newcommand{\Rbar}{\overline{\maji{R}}}
\newcommand{\RR}{\bigcat{R}}
\newcommand{\RRR}{\bigfun{R}}
\newcommand{\Rh}{\R_h}
\newcommand{\Rv}{\R_v}
\newcommand{\Rhv}{\R_{hv}}
\renewcommand{\S}{\maji{S}}
\renewcommand{\ss}{\bigcat{s}}
\renewcommand{\SS}{\bigcat{S}}
\newcommand{\SSS}{\bigfun{S}}
\newcommand{\SSSccs}{\bigfun{S}_{\Dccs}}
\newcommand{\SSn}{\SS_{[n]}}
\newcommand{\SSm}{\SS_{[m]}}
\newcommand{\SSni}{\SS_{[n']}}
\newcommand{\SSsing}{\SS^!}
\newcommand{\Ss}{\restr{S}{s}}
\newcommand{\SSX}{\SS_X}
\newcommand{\SSY}{\SS_Y}
\newcommand{\Sh}{\mathrm{Sh}}
\newcommand{\ShCEEh}{\Sh((\CE)_{\Eh})}
\newcommand{\ShCWEh}{\Sh((\W)_{\Eh})}
\newcommand{\StatesD}{\SSS_\D}
\newcommand{\CatPVEh}{\Cat(\PV_{\Eh})}
\newcommand{\mm}{\bigcat{m}} %
\newcommand{\ProcPVEh}{\Proc(\PV)}
\newcommand{\ProcPVEhsq}{\Proc(\PV)_{\Nat}}
\newcommand{\ProcPV}[1]{\Proc(\PV)_{#1}}
\newcommand{\ProcPVX}{\ProcPV{X}}
\newcommand{\ProcPVY}{\ProcPV{Y}}
\newcommand{\ProcEh}{\Proc{}}
\newcommand{\ProcoEh}{\Procoof{}}
\newcommand{\Procof}[1]{\Proc_{#1}}
\newcommand{\Procoof}[1]{\Proc^0_{#1}}
\newcommand{\ProcX}{\Procof{X}}
\newcommand{\ProcY}{\Procof{Y}}
\newcommand{\Shhat}{\hat{\Sh}}
\newcommand{\Sv}{\S_v}
\newcommand{\Svhat}{\hat{\Sv}}
\newcommand{\Shv}{\S_{\mathit{hv}}}
\newcommand{\Shvhat}{\hat{\S_{hv}}}
\newcommand{\T}{\maji{T}} %
\newcommand{\TT}{\bigcat{T}} %
\renewcommand{\tt}{\bigcat{t}} %
\newcommand{\TTT}{\bigfun{T}} %
\newcommand{\Th}{\T_h}
\newcommand{\Thw}{\T_h^\omega}
\newcommand{\Tv}{\T_v}
\newcommand{\Tvw}{\T_v^\omega}
\newcommand{\Thv}{\T_{hv}}
\newcommand{\Tree}{\bigcat{Tree}}
\newcommand{\Shat}{\hat{\S}}

\newcommand{\POSheaves}{\bigcat{POSh}}
\newcommand{\Occhat}{\hat{\Occ}}
\newcommand{\elhat}[1]{\widehat{\el #1}}
\newcommand{\flatten}{\maji{F}}
\newcommand{\Tw}{\T_\omega}
%\newcommand{\Sig}{\hat{\maji{S}}}
\newcommand{\Sig}{\bigcat{Sig}} %{\maji{S}}
\newcommand{\Sigcc}{\Sig_{\bigcat{cc}}} %{\maji{S}}
\newcommand{\StdSigi}{\bigcat{Sig}_{1}} 
\newcommand{\StdSig}{\bigcat{Sig}} 
\newcommand{\StoStdi}{\bigcat{U}_1}
\newcommand{\StoStdii}{\bigcat{U}_2}
\newcommand{\StdtoSi}{\bigcat{V}_1}
\newcommand{\StdtoSii}{\bigcat{V}_2}
\newcommand{\Typ}{\bigcat{Typ}}
\newcommand{\Set}{\bigcat{Set}}
\newcommand{\set}{\bigcat{set}}
\newcommand{\Rel}{\bigcat{Rel}}
\newcommand{\rel}{\bigcat{rel}}
\newcommand{\ford}{\bigcat{ford}}
\newcommand{\FinSet}{\bigcat{FinSet}}
\newcommand{\FinOrd}{\bigcat{FinOrd}}
\newcommand{\OPsh}[1]{\wideparen{#1}}
\newcommand{\FPsh}[1]{\overline{#1}}
\newcommand{\Pshf}[1]{\widehat{#1}^{{}_f}}
\newcommand{\Pshc}[1]{\widehat{#1}^{{}_c}}
\newcommand{\FinSetop}{\op\FinSet}
\newcommand{\Cpo}{\bigcat{Cpo}}
\newcommand{\PCpo}{\bigcat{PCpo}}
\newcommand{\MonPCpo}{\bigcat{Mon}(\PCpo)}
\newcommand{\CMonPCpo}{\bigcat{CMon}(\PCpo)}
\newcommand{\MonCpo}{\bigcat{Mon}(\Cpo)}
\newcommand{\CMonCpo}{\bigcat{CMon}(\Cpo)}
\newcommand{\Cat}{\bigcat{Cat}}
\newcommand{\MCat}{\bigcat{MonCat}}
\newcommand{\FPCat}{\bigcat{FPCat}}
\newcommand{\FPCatcc}{\bigcat{FPCat}_{\bigcat{cc}}}
\newcommand{\Mon}{\bigcat{Mon}}
\newcommand{\Kl}{\bigcat{Kl}}
\newcommand{\MCatcc}{\bigcat{MonCat}_{\bigcat{cc}}}
\newcommand{\TwoCat}{2\bigcat{Cat}}
\newcommand{\CCDCat}{\bigcat{CCDCat}}
\newcommand{\MCDCat}{\bigcat{MCDCat}}
\newcommand{\MCDCatcc}{\bigcat{MCDCat}_{\bigcat{cc}}}
\newcommand{\MDCat}{\bigcat{MonDCat}}
\newcommand{\CDCat}{\bigcat{CDCat}}
\newcommand{\CDCatcc}{\bigcat{CDCat}_{\bigcat{cc}}}
\newcommand{\MDCatcc}{\bigcat{MDCat}_{\bigcat{cc}}}
\newcommand{\CCat}{\bigcat{CCat}}
\newcommand{\MSig}{\bigcat{MonSig}}
\newcommand{\TMultiCat}{T\textrm{-}\bigcat{MultiCat}}
\newcommand{\TMultiCato}{T\textrm{-}\bigcat{MultiCat}_{\bigcat{o}}}
\newcommand{\TSpan}{T\textrm{-}\bigcat{Span}}
\newcommand{\TGph}{T\textrm{-}\bigcat{Gph}}

\newcommand{\fmcMultiCat}{\fmc\textrm{-}\bigcat{MultiCat}}
\newcommand{\fmcCMultiCat}{\fmc\textrm{-}\bigcat{CMultiCat}}
\newcommand{\fmcMultiCatcc}{\fmc\textrm{-}\bigcat{MultiCat}_{\bigcat{cc}}}
\newcommand{\fmcCMultiCatcc}{\fmc\textrm{-}\bigcat{CMultiCat}_{\bigcat{cc}}}
\newcommand{\fmcMultiCato}{\fmc\textrm{-}\bigcat{MultiCat}_{\bigcat{o}}}
\newcommand{\fmcSpan}{\fmc\textrm{-}\bigcat{Span}}
\newcommand{\fmcGph}{\fmc\textrm{-}\bigcat{Gph}}

\newcommand{\MMMultiCat}{\MM\textrm{-}\bigcat{MultiCat}}
\newcommand{\MMCMultiCat}{\MM\textrm{-}\bigcat{CMultiCat}}
\newcommand{\MMFPMultiCat}{\MM\textrm{-}\bigcat{FPMultiCat}}
\newcommand{\MMMultiCato}{\MM\textrm{-}\bigcat{MultiCat}_{\bigcat{o}}}
\newcommand{\MMSpan}{\MM\textrm{-}\bigcat{Span}}
\newcommand{\MMGph}{\MM\textrm{-}\bigcat{Gph}}

\newcommand{\CCCat}{\bigcat{CCCat}}
\newcommand{\MCCat}{\bigcat{MCCat}}
\newcommand{\QCat}{\Quintets{\Cat}}
\newcommand{\LinBotOrdf}{\bigcat{LOrd_{\bot,f}}}
\newcommand{\Proc}{\bigcat{Proc}}
\newcommand{\Procf}{\Proc_f}
\newcommand{\Gph}{\bigcat{Gph}}
\newcommand{\GCompl}{\bigcat{GCompl}}
\newcommand{\CCompl}{\bigcat{CCompl}}
\newcommand{\UCompl}{\bigcat{UCompl}}
\newcommand{\RGph}{\bigcat{RGph}}
\newcommand{\For}{\bigcat{For}}
\newcommand{\IGph}{\bigcat{IGph}}
\newcommand{\INat}{\mathbb{N}}
\newcommand{\INathat}{\widehat{\INat}}
\newcommand{\INatMx}{\INat / \M_x}
\newcommand{\INatMn}{\INat / \M_n}
\newcommand{\Mod}{\bigcat{Mod}}
\newcommand{\CAT}{\bigcat{CAT}}
\newcommand{\CCAT}{\bigcat{CAT}_d}
\newcommand{\Top}{\bigcat{Top}}
\newcommand{\DTop}{\bigcat{DTop}}
\newcommand{\Setp}{\bigcat{Setp}}
\newcommand{\SMCCat}{\bigcat{SMCCat}}
\newcommand{\SSMCat}{\bigcat{SSMCat}}
\newcommand{\ccset}{\bigcat{CCSet}}
\newcommand{\cccat}{\bigcat{CCCat}}
\newcommand{\ccth}{\bigcat{CCTh}}
\newcommand{\bth}{\bigcat{BTh}_{\mathrm{HM}}}
\newcommand{\Bth}{\bigcat{BTh}}
\newcommand{\CCS}{\mathit{CCS}}
\newcommand{\CCSsig}{F_\mathit{CCS}}
\newcommand{\SLin}{\bigcat{SLin}}
\newcommand{\usualth}{\bigcat{Th}}
\newcommand{\ccmcat}{\bigcat{CCMCat}}
\newcommand{\tcccat}{\bigcat{2CCCat}}
\newcommand{\tccmcat}{\bigcat{2CCMCat}}
\newcommand{\End}{\bigcat{End}}
\newcommand{\Shapely}{\bigcat{Shap}}
\newcommand{\Tight}{\bigcat{Tight}}
\newcommand{\RTight}{\bigcat{Tight}_\R}
\newcommand{\occ}{\xi}
\newcommand{\piget}{\ensuremath{\mathit{g}}}
\newcommand{\pisend}{\ensuremath{\mathit{s}}}
\newcommand{\trou}{\boxempty}
\newcommand{\vercomp}{\mathbin{\bullet}}
\newcommand{\inclh}{\iota_h}
\newcommand{\inclv}{\iota_v}
\newcommand{\colimP}{\check{P}}
\newcommand{\elcolimP}{\el\colimP}
\DeclareMathOperator{\sk}{\mathrm{skel}}
\newcommand{\Fib}{\bigcat{Fib}}
\newcommand{\DFib}{\bigcat{DFib}}
\newcommand{\fib}[1]{\widetilde {#1}}
\newcommand{\FibOcco}{\fib \Occo}
\newcommand{\FibOcci}{\fib \Occi}
\newcommand{\FibSi}{\fib \Si}
\newcommand{\FibS}{\fib \S}
\newcommand{\Fibun}{\fib 1}
\newcommand{\Inj}{\bigcat{Inj}}

% vocabulary
\newcommand{\ty}{\textsf{ty}}
\newcommand{\Nat}{\mathbb{N}} % set of natural numbers
\newcommand{\smc}{\textsc{smc}}
\newcommand{\hors}{\textsc{hors}}
\newcommand{\horses}{\textsc{hors}es}
\newcommand{\ccc}{\textsc{ccc}}
\newcommand{\ccmc}{\textsc{ccmc}}
\newcommand{\tccc}{cartesian closed 2-category}
\newcommand{\tcccs}{cartesian closed 2-categories}
\newcommand{\tccmc}{\textsc{2ccmc}}
\newcommand{\ccts}{cartesian closed 2-signature}
\newcommand{\cctss}{cartesian closed 2-signatures}
\newcommand{\Ccts}{Cartesian closed 2-signature}
\newcommand{\Cctss}{Cartesian closed 2-signatures}
\newcommand{\rreduction}{rreduction}
\newcommand{\rreductions}{rreductions}
\newcommand{\Rreduction}{Rreduction}
\newcommand{\Rreductions}{Rreductions}
\newcommand{\ssm}{\textsc{ssm}}
\newcommand{\ssmc}{\textsc{ssmc}}
\newcommand{\lra}{\textsc{lra}}
\newcommand{\dr}{\textsc{dr}}
\newcommand{\hoas}{\textsc{hoas}}
\newcommand{\imll}{\textsc{imll}}
\newcommand{\fst}{\mathtt{i}_1}
\newcommand{\snd}{\mathtt{i}_2}
\newcommand{\abs}{\ell}
\newcommand{\app}{a}
\newcommand{\sexp}{\emph{sexp}}
\newcommand{\loc}{\ell}
\newcommand{\prnt}{\mathit{prnt}}
\newcommand{\link}{\mathit{link}}
\newcommand{\ctrl}{\mathit{ctrl}}
\newcommand{\var}{\mathit{var}}
\newcommand{\prt}{\mathit{prt}}
\newcommand{\lnk}{\mathit{lnk}}
\newcommand{\aux}{\mathit{aux}}
\newcommand{\pri}{\mathit{pri}}
\newcommand{\bin}{\mathit{bin}}
\newcommand{\MonL}{\fonc{Mon}(\Lambda)}
\newcommand{\ModL}{\fonc{Mod}(\Lambda)}
\newcommand{\LC}{\fonc{LC}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\un}{1}
\newcommand{\para}{\mathbin{\mid}}
\newcommand{\thg}{{\mathord{\text{--}}}}
\newcommand{\shape}[2]{[#1, #2]}
\newcommand{\transli}[1]{\lsem #1 \rsem'}
\newcommand{\transl}[1]{\lsem #1 \rsem}
\newcommand{\translfun}{\lsem - \rsem}
\newcommand{\Transl}[1]{\llparenthesis #1 \rrparenthesis}
\newcommand{\Translfun}{\Transl{-}}
\newcommand{\translun}[1]{\lsem #1 \rsem^1}
\newcommand{\transldeux}[1]{\lsem #1 \rsem^2}
\newcommand{\transltrois}[1]{\lsem #1 \rsem^3}
% maths
\newcommand{\rond}{\circ}
\newcommand{\vrond}{\mathbin{\bullet}}
\newcommand{\vcompose}[1]{#1^{\vrond}}
\newcommand{\vcomposefun}{(-)^{\vrond}}
\newcommand{\vcomposeH}[1]{#1^{\vrond}}
\newcommand{\vcomposeHfun}{(-)_H^{\vrond}}
\newcommand{\bsquare}{\mathbin{\scriptstyle \blacksquare}}
\newcommand{\id}{\mathit{id}}
\newcommand{\idv}{\mathit{id}^{\vrond}}
\newcommand{\oneH}{\mathbf{1}}
\newcommand{\iso}{\cong}
\newcommand{\niso}{\ncong}
\newcommand{\impll}{\multimap}
\newcommand{\tens}{\otimes}
\newcommand{\bigtens}{\bigotimes}
\newcommand{\Bigtens}[1]{\displaystyle{\bigtens_{#1}}}
\newcommand{\Bigcup}[1]{\displaystyle{\bigcup_{#1}}}
\newcommand{\Union}[1]{\Bigcup{#1}}
\newcommand{\mycoprod}{\sum}
\newcommand{\Coprod}[1]{\displaystyle{\mycoprod_{#1}}}
%\newcommand{\coprod}[1]{\mycoprod_{#1}}
\newcommand{\Prod}[1]{\displaystyle{\prod_{#1}}}
\newcommand{\inj}{\mathit{inj}}
\newcommand{\push}[1]{\mathbin{+_{#1}}}
\newcommand{\pull}[1]{\mathbin{\times_{#1}}}
\newcommand{\card}[1]{|#1|}
\newcommand{\base}[1]{|#1|}
\newcommand{\eqdef}{\stackrel{\mathtt{def}}{=}}
\newcommand{\eq}{\mathrel{\texttt{:=}}}
\newcommand{\ens}[1]{\{ #1 \}}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\aalt}{\mathrel{|}}
\newcommand{\name}[1]{\ulcorner #1 \urcorner}
\newcommand{\op}[1]{#1^{\mathit{op}}}
\newcommand{\nop}[1]{#1^{\bot}}
%\newcommand{\notbot}{\not {\mathord{\bot\ }}}
\newcommand{\send}[2]{\ensuremath{\bar{#1}\langle#2\rangle}}
\newcommand{\sendab}{\send{a}{b}}
\newcommand{\get}[2]{\ensuremath{#1(#2)}}
\newcommand{\alphabar}{\bar{\alpha}}
\newcommand{\lam}{\ensuremath{\lambda}}
\newcommand{\Lam}{\ensuremath{\Lambda}}
\newcommand{\LamCats}{\ensuremath{\lam\mbox{-}\bigcat{Cat}_s}}
\newcommand{\DbCat}{\ensuremath{\bigcat{DbCat}}}
\newcommand{\ver}[2]{\langle#1, #2\rangle}
\newcommand{\pairing}[2]{\langle#1, #2\rangle}
\newcommand{\tupling}[1]{\langle #1 \rangle}
\newcommand{\downwardsPairing}[2]{{/}#1, #2{\backslash}}
\newcommand{\chan}[1]{\langle#1\rangle}
\newcommand{\ABCD}{\begin{diagram}[inline,width=1em,height=1em]
          A & B \\
          C & D
        \end{diagram}}
\newcommand{\hijk}{\begin{diagram}[inline,width=1em,height=1em]
          h & i \\
          j & k
        \end{diagram}}

\newcommand{\Quintets}[1]{\mathbb{Q}#1}
\newcommand{\shap}[2]{(#1,#2)}
\newcommand{\subs}[1]{[#1]}
\newcommand{\Talg}{\Shat^T}
\newcommand{\Thwalg}{\mbox{$\Thw$-alg}}
\newcommand{\Synt}{\maji{H}}
\newcommand{\Syntv}{\maji{V}}
\newcommand{\SSMCCats}{\bigcat{SSMCCat}}
\newcommand{\Soup}{\comate \coma \S}
\newcommand{\coma}{{\sslash}}
\newcommand{\faithslash}{\mathbin{/_{\! \! \! f}}}
\newcommand{\comate}{S}
\newcommand{\plonge}{\iota}
\newcommand{\dstar}{d^\star}
\newcommand{\drond}{d^\circ}
\newcommand{\cstar}{c^\star}
\newcommand{\sstar}{s^\star}
\newcommand{\crond}{c^\circ}
\newcommand{\srond}{s^\circ}
\newcommand{\wstar}{w^\star}
\newcommand{\wrond}{w^\circ}
\newcommand{\lamapp}{\lam\app}
\newcommand{\deltarond}{\delta^{\circ}}
\newcommand{\expleaf}[2]{{#1}^{\langle #2 \rangle}}
\newcommand{\expleafn}[1]{\expleaf{#1}{n}}
\newcommand{\unweave}{\nabla}
\newcommand{\deltad}{\delta_d}
\newcommand{\epsilond}{\epsilon_d}
\newcommand{\ev}{\mathit{ev}}
\newcommand{\evI}{\ev_I}
\newcommand{\evM}{\ev_M}
\newcommand{\evC}[1]{\lsem #1 \rsem_{\C}}
\newcommand{\evCfun}{\lsem - \rsem_{\C}}
\newcommand{\Gam}{\Gamma}
\newcommand{\gam}{\gamma}
\newcommand{\Del}{\Delta}
\newcommand{\del}{\delta}
\newcommand{\EM}{E}
\newcommand{\nt}{\mathrel{\uparrow}}
\newcommand{\nf}{\mathrel{\downarrow}}
\newcommand{\ut}{\mathrel{:::}}
\newcommand{\elt}{\mathrm{b}}
\newcommand{\labelD}{\ell_\D}
\newcommand{\labelDW}{\ell_\D^\W}

\newcommand{\labelDccs}{\ell_{\D}}
\newcommand{\labelDccsW}{\ell_{\Dccs}^\W}
\newcommand{\labelDccsfunctor}{\bar{\ell}_{\D}}
\newcommand{\labelDccsfunctorW}{\bar{\ell}_{\Dccs}^\W}

\newcommand{\either}{\mathrel{::}}
\newcommand{\rcolon}{\mathrel{:}}
\newcommand{\red}{\mathrel{\to}}
\newcommand{\redof}[2]{\mathrel{\xrightarrow{#1}_{#2}}}
\newcommand{\redPV}{\redof{V}{\P}}
\newcommand{\rred}{\mathrel{\leadsto}}
\newcommand{\rredcon}{\mathrel{\rred_{\mathit{con}}}} 
\newcommand{\rredsim}{\mathrel{\rred_{\mathit{sim}}}} 
\newcommand{\rredcom}{\mathrel{\rred_{\mathit{com}}}} 
\newcommand{\rredper}{\mathrel{\rred_{\mathit{per}}}} 
\newcommand{\rredlif}{\mathrel{\rred_{\mathit{lif}}}}
\newcommand{\rredlifsim}{\mathrel{\rred_{\mathit{lif}, \mathit{sim}}}} 
\newcommand{\req}{\mathrel{\equiv}}
\newcommand{\equi}{\simeq}
\newcommand{\wbisim}{\mathrel{\approx}}
\newcommand{\bisim}{\mathrel{\sim}}
\newcommand{\wbisimA}{\mathrel{\wbisim_\A}}
\newcommand{\wbisima}{\mathrel{\wbisim_A}}
\newcommand{\wbisimsierp}{\mathrel{\wbisim_\Sierp}}
\newcommand{\bisimsierp}{\mathrel{\bisim_\Sierp}}
\newcommand{\iotawbisim}{\mathrel{\wbisim_{\tau,\iota}}}
\newcommand{\iotabisim}{\mathrel{\wbisim_{\iota}}}
\newcommand{\iotawbisimo}{\mathrel{\wbisim_{\tau,\iota}^0}}
\newcommand{\iotawbisimI}{\mathrel{\wbisim_{\tau,\iota}^I}}
\newcommand{\iotawbisimIo}{\mathrel{\wbisim_{\tau,\iota}^{I,0}}}
\newcommand{\inducedeq}{\mathrel{\inv{\transl{\faireq}}}}
\newcommand{\sigmabisim}{\mathrel{\simeq_{\sigma}}}

\newcommand{\faireq}{\mathrel{\sim_f}}
%\newcommand{\faireqg}{\mathrel{\sim}}
\newcommand{\fairneq}{\mathrel{\nsim_f}}
\newcommand{\faireqs}{\mathrel{\sim_{f,s}}}
%\newcommand{\faireqA}{\mathrel{\sim_{f,\A}}}
%\newcommand{\fairneqA}{\mathrel{\nsim_{f,\A}}}
\newcommand{\vcomp}[1]{\mathbin{;_{#1}}}
\newcommand{\proj}{\pi}
\newcommand{\projj}{\pi'}
\newcommand{\canonic}{i}
\newcommand{\skel}[1]{\lfloor #1 \rfloor}
\newcommand{\skelfun}{\lfloor \cdot \rfloor}
\newcommand{\Lamo}{\ensuremath{\Lambda_0}}
\newcommand{\Lo}{\ensuremath{\L_0}}
\newcommand{\So}{\ensuremath{\S_0}}
\newcommand{\To}{\ensuremath{\T_0}}
\newcommand{\Occo}{\ensuremath{\Occ_0}}
\newcommand{\Sohat}{\hat{\So}}
\newcommand{\Soop}{\op{\So}}
\newcommand{\Occoop}{\op{\Occo}}
\newcommand{\Tohat}{\hat{\To}}
\newcommand{\Occohat}{\hat{\Occo}}
\newcommand{\Occosm}{\Occo'}
\newcommand{\Occosmhat}{\hat{\Occosm}}
\newcommand{\jo}{j_0}
\newcommand{\ji}{j_1}
\newcommand{\Occism}{\Occi'}
\newcommand{\Occismhat}{\hat{\Occism}}
\newcommand{\Li}{\ensuremath{\L_1}}
\newcommand{\Si}{\ensuremath{\S_1}}
\newcommand{\Ti}{\ensuremath{\T_1}}
\newcommand{\Occi}{\ensuremath{\Occ_1}}
\newcommand{\Lami}{\ensuremath{\Lam_1}}
\newcommand{\Sihat}{\hat{\Si}}
\newcommand{\Siop}{\op{\Si}}
\newcommand{\Occiop}{\op{\Occi}}
\newcommand{\Tihat}{\hat{\Ti}}
\newcommand{\Occihat}{\hat{\Occi}}
\newcommand{\Lii}{\ensuremath{\L_2}}
\newcommand{\Sii}{\ensuremath{\S_2}}
\newcommand{\Tii}{\ensuremath{\T_2}}
\newcommand{\Occii}{\ensuremath{\Occ_2}}
\newcommand{\Lamii}{\ensuremath{\Lam_2}}
\newcommand{\Siihat}{\hat{\Sii}}
\newcommand{\Siiop}{\op{\Sii}}
\newcommand{\Occiiop}{\op{\Occii}}
\newcommand{\Tiihat}{\hat{\Tii}}
\newcommand{\Occiihat}{\hat{\Occii}}
\newcommand{\jii}{j_2}
\newcommand{\Eta}{\eta}
\newcommand{\monadify}{m}
\newcommand{\cga}{c_{(G,A)}}
\newcommand{\cpiga}{c_{(\prod G,A)}}
\newcommand{\vermn}{\ver{M}{N}}

\newcommand{\STo}{\mathit{st}_0}
\newcommand{\SOo}{\mathit{so}_0}
\newcommand{\OSo}{\mathit{os}_0}
\newcommand{\OOo}{\mathit{oo}_0}
\newcommand{\TOo}{\mathit{to}_0}
\newcommand{\STi}{\mathit{st}_1}
\newcommand{\SOi}{\mathit{so}_1}
\newcommand{\OSi}{\mathit{os}_1}
\newcommand{\OOi}{\mathit{oo}_1}
\newcommand{\TOi}{\mathit{to}_1}
\newcommand{\OToi}{\mathit{ot}_{01}}
\newcommand{\SSoi}{\mathit{ss}_{01}}
\newcommand{\SToi}{\mathit{st}_{01}}
\newcommand{\OTiii}{\mathit{ot}_{12}}
\newcommand{\SSiii}{\mathit{ss}_{12}}
\newcommand{\STii}{\mathit{st}_2}
\newcommand{\ruleset}[2]{
%\mbox{#1}\hrulefill
{\ } \\
\mbox{#1} \\ \hrulefill
  \begin{mathpar}
    #2
  \end{mathpar}
}
\newcommand{\bureaucratic}[1]{}
%\def\bbar{{\mathchar'26\mkern-9mu b}} 
\newcommand{\nonid}[1]{\bbar \ens{#1}}
\newcommand{\abar}{\overline{a}}
\newcommand{\bbar}{\overline{b}}
\newcommand{\ibar}{\overline{i}}
\newcommand{\onebar}{\overline{1}}
\newcommand{\sender}{\epsilon}
\newcommand{\receiver}{\rho}
\newcommand{\LAlg}{\L\mbox{-}\mathrm{Alg}}
\newcommand{\LiAlg}{\L_1\mbox{-}\mathrm{Alg}}

\newcommand{\namen}[1]{s_{#1}}
\newcommand{\cioio}{\iota}
\newcommand{\iotaof}[2]{\iota_{#1,#2}}
\newcommand{\iotani}{\iotaof{n}{i}}
\newcommand{\ciopos}{o}
\newcommand{\cioneg}{\iota}
\newcommand{\iotapos}[1]{o_{#1}}
\newcommand{\iotaneg}[1]{\iota_{#1}}
\newcommand{\iotaposni}{\iotapos{n,i}}
\newcommand{\iotaposmj}{\iotapos{m,j}}
\newcommand{\iotaposnj}{\iotapos{n,j}}
\newcommand{\iotanegni}{\iotaneg{n,i}}
\newcommand{\iotanegmj}{\iotaneg{m,j}}
\newcommand{\iotanegnj}{\iotaneg{n,j}}
\newcommand{\paraof}[1]{\pi_{#1}}
\newcommand{\paral}{\paralof{}}
\newcommand{\parar}{\pararof{}}
\newcommand{\paralof}[1]{\pi^l_{#1}}
\newcommand{\pararof}[1]{\pi^r_{#1}}
\newcommand{\paran}{\paraof{n}}
\newcommand{\paraln}{\paralof{n}}
\newcommand{\pararn}{\pararof{n}}
\newcommand{\parap}{\paraof{p}}
\newcommand{\paralp}{\paralof{p}}
\newcommand{\pararp}{\pararof{p}}
\newcommand{\paragam}{\paraof{\Gam}}
\newcommand{\paralgam}{\paralof{\Gam}}
\newcommand{\parargam}{\pararof{\Gam}}
\newcommand{\parazero}{\paraof{0}}
\newcommand{\paraofij}[2]{\mathbin{{}_{#1}\!\para\!{}_{#2}}}
\newcommand{\paraij}{\paraofij{i}{j}}
\newcommand{\paraundeux}{\paraofij{1}{2}}
\newcommand{\paradeuxun}{\paraofij{2}{1}}
\newcommand{\cparaof}[1]{\paraof{#1}^0}
\newcommand{\cparan}{\cparaof{n}}
\newcommand{\epara}{e^{\paraof{}}}
\newcommand{\cparalof}[1]{\paraof{#1}^{l_0}}
\newcommand{\cparaln}{\cparalof{n}}
\newcommand{\eparal}{e^{\paralof{}}}
\newcommand{\cpararof}[1]{\paraof{#1}^{r_0}}
\newcommand{\cpararn}{\cpararof{n}}
\newcommand{\ecpararn}{e^{\cpararn}}
\newcommand{\ecparaln}{e^{\cparaln}}
\newcommand{\nuof}[1]{\nu_{#1}}
\newcommand{\nun}{\nuof{n}}
\newcommand{\nup}{\nuof{p}}
\newcommand{\nugam}{\nuof{\Gam}}
\newcommand{\tickof}[1]{\tick_{#1}}
\newcommand{\tickn}{\tickof{n}}
\newcommand{\tickp}{\tickof{p}}
\newcommand{\tickgam}{\tickof{\Gam}}
\newcommand{\tauof}[4]{\tau_{#1,#2,#3,#4}}
\newcommand{\taunimj}{\tauof{n}{i}{m}{j}}
\newcommand{\taumjni}{\tauof{m}{j}{n}{i}}
\newcommand{\taunimjk}{\tau_{n,i,m,j,k}}
\newcommand{\taunamcd}{\tau_{n,a,m,c,d}}
\newcommand{\taunlmjk}{\tau_{n,l,m,j,k}}
\newcommand{\horn}{\tau^-}
\newcommand{\hornof}[4]{\horn_{#1,#2,#3,#4}}
\newcommand{\hornnimj}{\hornof{n}{i}{m}{j}}
\newcommand{\skelof}[1]{#1^-}
\newcommand{\cores}[1]{\mathrm{cores} (#1)}
\newcommand{\core}[1]{\mathrm{core} (#1)}
\newcommand{\skeltaunimj}{\tau^0_{n,i,m,j}}
\newcommand{\strip}[1]{\llcorner #1 \lrcorner}
\newcommand{\stripfun}{\strip{-}}
\newcommand{\States}[1]{\mathrm{States} (#1)}
\newcommand{\Elfun}{\mathrm{El}}
\newcommand{\El}[1]{\Elfun (#1)}
\newcommand{\SynF}{\bigcat{F}}
\newcommand{\derivmap}{\bigcat{d}}

\newcommand{\diagapp}{ \diag(1.2,1.2){
    \&  \& |(MN)| MN \\
    \&     \&              |(M)| M     \&  |(N)| N\\
    \& |(GB)| (G,B) \& |(GBA)| (G, B^A) \& |(GA)| (G, A) \\
    |(G)| G \& \& |(BA)| B^A \& \\
    \& |(B)| B \& \& |(A)| A }{ (GB) edge (MN) %
    (GBA) edge (M) %
    (GA) edge (N) %
    (M) edge (MN) %
    (N) edge (MN) %
    (B) edge (GB) %
    (BA) edge (GBA) %
    (A) edge (GA) %
    (B) edge (BA) %
    (A) edge (BA) %
    (G) edge [background] (GA) edge [background] (GBA) edge
    [background] (GB) %
    edge (GA) edge (GBA) edge (GB) %
  } } 

\newcommand{\PV}{\pow (\V)}
\newcommand{\PVX}{\pow (\V)_X}
\newcommand{\PVY}{\pow (\V)_Y}
\newcommand{\Up}{\mathrm{Up}}
\newcommand{\Sq}{\mathrm{Sq}}
\newcommand{\Pl}{\mathrm{Pl}}
\newcommand{\PlB}{\Pl_{\DB}}
%\newcommand{\precsim}[1]{\prec_{\sim_{#1}}}
\newcommand{\precsimU}{\precsim_{U}}
\newcommand{\Paths}[1]{\Pathsfun (#1)}
\newcommand{\Pathsfun}{N_{\M_x}}
\newcommand{\LanJop}{\Lan_{\op\J}}
\newcommand{\RanJop}{\Ran_{\op\J}}
\newcommand{\LanKop}{\Lan_{\op\K}}
\newcommand{\RanKop}{\Ran_{\op\K}}
\newcommand{\RanKopSh}{\RanKop^\mathrm{Sh}}
\newcommand{\Pathsover}[1]{\widehat{\INat / \M_{#1}}}
\newcommand{\LTSfun}{\bigcat{LTS}}
\newcommand{\LTS}[1]{\LTSfun_{#1}}
\newcommand{\lts}{\textsc{lts}}
\newcommand{\anlts}{an \lts{}}
\newcommand{\ltss}{\lts{s}}
\newcommand{\Lts}{\textsc{Lts}}
\newcommand{\Ltss}{\Lts{s}}

\newcommand{\action}{action\xspace}
\newcommand{\anaction}{an action\xspace}
\newcommand{\actions}{actions\xspace}
\newcommand{\Action}{Action\xspace}
\newcommand{\Anaction}{An action\xspace}
\newcommand{\Actions}{Actions\xspace}

\newcommand{\agent}{agent\xspace}
\newcommand{\anagent}{an agent\xspace}
\newcommand{\agents}{agents\xspace}
\newcommand{\Agent}{Agent\xspace}
\newcommand{\Anagent}{An agent\xspace}
\newcommand{\Agents}{Agents\xspace}

\newcommand{\thread}{view\xspace}
\newcommand{\athread}{a view\xspace}
\newcommand{\threads}{views\xspace}
\newcommand{\Thread}{View\xspace}
\newcommand{\Athread}{A view\xspace}
\newcommand{\Threads}{Views\xspace}

\newcommand{\configuration}{configuration\xspace}
\newcommand{\aconfiguration}{a configuration\xspace}
\newcommand{\configurations}{configurations\xspace}
\newcommand{\Configuration}{Configuration\xspace}
\newcommand{\Aconfiguration}{A configuration\xspace}
\newcommand{\Configurations}{Configurations\xspace}
\newcommand{\subconfiguration}{subconfiguration\xspace}
\newcommand{\subconfigurations}{subconfigurations\xspace}
\newcommand{\Subconfigurations}{Subconfigurations\xspace}

\newcommand{\trace}{trace\xspace}
\newcommand{\atrace}{a trace\xspace}
\newcommand{\traces}{traces\xspace}
\newcommand{\Trace}{Trace\xspace}
\newcommand{\Atrace}{A trace\xspace}
\newcommand{\Traces}{Traces\xspace}

\newcommand{\stratglobale}{strategy\xspace}
\newcommand{\astratglobale}{a strategy\xspace}
\newcommand{\stratglobales}{strategies\xspace}
\newcommand{\Stratglobale}{Strategy\xspace}
\newcommand{\Astratglobale}{A strategy\xspace}
\newcommand{\Stratglobales}{Strategies\xspace}

\newcommand{\stratlocale}{behaviour\xspace}
\newcommand{\astratlocale}{a behaviour\xspace}
\newcommand{\stratlocales}{behaviours\xspace}
\newcommand{\Stratlocale}{Behaviour\xspace}
\newcommand{\Astratlocale}{A behaviour\xspace}
\newcommand{\Stratlocales}{Behaviours\xspace}


\newcommand{\Moves}{\bigcat{Moves}}
\newcommand{\FCMoves}{\bigcat{FCMoves}} 
\newcommand{\CMoves}{\bigcat{CMoves}}
\newcommand{\prefixed}{\mathrm{prefixed}}
\newcommand{\program}{\mathrm{program}}
\newcommand{\orth}{\pitchfork}
\newcommand{\ortho}{\mathrel{\bot}}
\newcommand{\orthright}[1]{#1^{\orth}}
\newcommand{\orthleft}[1]{{{}^{\orth}#1}}
\newcommand{\botright}[1]{#1^{\bot}}
\newcommand{\botleft}[1]{{{}^{\bot}#1}}
\newcommand{\botrightleft}[1]{\botleft{(\botright{#1})}}
\newcommand{\botleftright}[1]{\botright{(\botleft{#1})}}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}} 
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}} 
\newcommand{\bbot}{\mathord{\independent}}
% \def\barebotT#1{\mathrel{\text{\rlap{$#1\sim$}$\mkern2mu{#1|}$}}}
% \newcommand{\barebot}{\protect\mathpalette{\protect\barebotT}}
\newcommand{\barebot}{\simperp}
\newcommand{\bbotmay}{\bbot^{\mathit{may}}}
\newcommand{\bbotmust}{\bbot^{\mathit{m}}}
\newcommand{\bbotfair}{\bbot^{\mathit{f}}}
\newcommand{\bbotfairi}{\bbot^{\mathit{f}'}}
\newcommand{\bbotmays}{\bbot^{\mathit{may},s}}
\newcommand{\bbotmusts}{\bbot^{\mathit{m},s}}
\newcommand{\bbotfairs}{\bbot^{\mathit{f},s}}
\newcommand{\bbotfairis}{\bbot^{\mathit{f}',s}}
\newcommand{\daimon}{\heartsuit}
\newcommand{\precUV}{\mathrel{\prec^V_U}}
\newcommand{\precWV}{\mathrel{\prec^V_W}}
\newcommand{\precUU}{\mathrel{\prec^U_U}}
\newcommand{\precu}{\mathrel{\prec_u}}
\newcommand{\simultaneous}{\Join}
\newcommand{\trtwo}[1]{\tr_2 (#1)}
\DeclareMathOperator{\close}{close}
\newcommand{\accepted}{\mathbf{Acc}}
\newcommand{\moveof}[2]{#1.#2}
\newcommand{\context}[3]{#3 \cdot (#1, #2)}
\newcommand{\letin}[2]{\texttt{let}\ #1\ \texttt{in}\ #2}
\newcommand{\recin}[2]{\texttt{rec}\ #1\ \texttt{in}\ #2}
\newcommand{\Gl}{\GG}
\newcommand{\GlX}{\Gl_X}
\newcommand{\glue}{\parallel}
\newcommand{\SStoGG}{\bigcat{Gl}}
\newcommand{\waiting}[1]{\bigcat{w} (#1)}
\newcommand{\activ}[1]{\activfun (#1)}
\newcommand{\activfun}{\mathrm{active}}
\newcommand{\state}{\sigma}
\newcommand{\statei}{\sigma'}
\newcommand{\stateii}{\sigma''}
\newcommand{\down}{\mathord{\downarrow}}
\newcommand{\baseof}[1]{\lfloor #1 \rfloor}
\newcommand{\Comoves}{\bigcat{CoMoves}}
\newcommand{\Degstart}[1]{\mathrm{Deg}_t (#1)}
\newcommand{\Degend}[1]{\mathrm{Deg}_s (#1)}
\newcommand{\DegM}[1]{\mathrm{Deg}_M (#1)}
\newcommand{\Basictwo}[1]{\mathrm{BM}_{#1}}
\newcommand{\dEsc}{\mathrm{d}}
\newcommand{\propagate}{\mathrm{p}}
\newcommand{\unfold}{\mathrm{unfold}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\deriv}{\partial}
\newcommand{\border}{\partial}
\newcommand{\may}{\mathit{may}}
\newcommand{\ec}{\bigcat{e}}
\newcommand{\eci}{\bigcat{f}}
\newcommand{\ecii}{\bigcat{g}}
\newcommand{\TCont}{\mathrm{TCont}}
\newcommand{\Evcont}{\mathrm{Evcont}}
\newcommand{\new}{\nu}
\newcommand{\as}{A}
\newcommand{\RS}{\bigcat{RS}}
\newcommand{\RG}{\bigcat{RG}}
\newcommand{\SR}{\bigcat{SR}}
\newcommand{\SG}{\bigcat{SG}}
\newcommand{\eof}{\mathit{eof}}
\newcommand{\ok}{\mathit{ok}}
\newcommand{\okbar}{\overline{\ok}}
\newcommand{\restart}{\mathit{restart}}
\newcommand{\restartbar}{\overline{\restart}}
\newcommand{\LLH}{\bigfun{L}}
\newcommand{\RRH}{\bigfun{R}}
\newcommand{\extfunfun}{\bigcat{ext}}
\newcommand{\extfun}[1]{\extfunfun_{#1}}
\newcommand{\ext}[2]{\extfun{#1} (#2)}
\newcommand{\exta}[2]{\overline{#2}}
\newcommand{\extafun}[1]{\overline{(-)}}
\newcommand{\uclose}[2]{#1 \uparrow #2}
\newcommand{\past}[1]{\mathrm{past} (#1)}
\newcommand{\Decomp}[1]{\bigcat{D}_{#1}}
\newcommand{\length}[1]{|#1|}
\newcommand{\Exonze}{\mathrm{Ex}_{11}}
\newcommand{\Sierp}{\Sigma}
\newcommand{\pbang}[2]{#1_{!}(#2)}
\newcommand{\pbangfun}[1]{#1_!}
\newcommand{\cw}[1]{\pbang{{\labelDW}}{#1}}
\newcommand{\cwA}[1]{\pbang{{\labelA}}{#1}}
\newcommand{\cwfun}{\pbangfun{{\labelDW}}}
\newcommand{\gluealong}[2]{\mathbin{{}_{#1}|_{#2}}}
\newcommand{\pbkchi}[1]{#1^\LLL}
\newcommand{\SSSI}{\SSS^I}
\newcommand{\TTTI}{\TTT^I}
\newcommand{\SSSDI}{\SSS^I_\D}
\newcommand{\TTTDI}{\TTT^I_\D}
\newcommand{\SSSL}{\pbkchi{\SSS}}
\newcommand{\SSSLlocal}{\pbkchi{\SSS}_{\mathrm{local}}}
\newcommand{\SSSind}{\pbkchi{\SSS}_{\mathrm{ind}}}
\newcommand{\SSSrho}{\SSS^\rho}
\newcommand{\TTTL}{\pbkchi{\TTT}}
\newcommand{\rc}[1]{#1^\A}
\newcommand{\SSSA}{\rc{\SSS}}
\newcommand{\TTTA}{\rc{\TTT}}
\newcommand{\SSSAccs}{\rc{\SSS_{\Dccs}}}
\newcommand{\TTTAccs}{\rc{\TTT_{\Dccs}}}
\newcommand{\pchifun}{p_\chi}
\newcommand{\pchi}[1]{\pchifun(#1)}
\newcommand{\failoffun}{\mathbf{fl}}
\newcommand{\failof}[1]{\failoffun(#1)}
\newcommand{\testable}[1]{#1^{\coh}}
\newcommand{\eqtestable}[2]{#1 \bowtie #2}
\newcommand{\GC}{\bigcat{GC}}
\newcommand{\LGC}{\bigcat{LGC}}
\newcommand{\scong}{\mathrel{\equiv}}

\tikzset{history/.style = {-open triangle 45}}
\newcommand{\xhistto}[1]{\mathbin{\tikz[baseline] \draw (0pt,.5ex) edge[history,labelu={\scriptstyle #1}] (3ex,.5ex);}}
\newcommand{\histto}{\xhistto{}}

\newcommand{\bambof}[1]{\langle #1 \rangle}
\newcommand{\bambn}{\bambof{n}}
\newcommand{\bambm}{\bambof{m}}
\newcommand{\botrel}{\mathrel{\bot}}
\newcommand{\rhorel}{\mathrel{\rho}}
\newcommand{\gamrel}{\mathrel{\gamma}}
\newcommand{\nbotrel}{\mathrel{\notbot}}
\newcommand{\botrelA}{\mathrel{\bot_\A}}
\newcommand{\nbotrelA}{\mathrel{\notbot_\A}}
\newcommand{\botA}{\bot_\A}
\newcommand{\xhatto}[1]{\xto{\widehat{#1}}}
\newcommand{\xhatot}[1]{\xot{\widehat{#1}}}
\newcommand{\idfree}[1]{\widetilde{#1}}
%\newcommand{\vdashdefinite}{\vdash_{\mathsf{D}}}
\def\vdashdefinitesymb{{\vdash\mkern-12mu{}_{\scriptscriptstyle \mathsf{D}}}}
\newcommand{\vdashdefinite}{\mathrel{\vdashdefinitesymb}}
%\newcommand{\vdashdefinite}{\underset{\raisebox{.7em}{\hspace*{-.3em}{\scriptscriptstyle \mathsf{D}}}}{\vdash}}
\newcommand{\vecteur}[2]{#1_1, \ldots, #1_{#2}}
\newcommand{\vecteurn}[1]{\vecteur{#1}{n}}
\newcommand{\vecteurnalpha}[1]{\vecteur{#1}{n_\alpha}}
\newcommand{\vecteurp}[1]{\vecteur{#1}{p}}

\newcommand{\outof}[3]{o_{#1,#2,#3}}
\newcommand{\outnjk}{o_{n,j,k}}
\newcommand{\outnij}{o_{n,i,j}}
\newcommand{\outnil}{o_{n,i,l}}
\newcommand{\outnab}{o_{n,a,b}}
\newcommand{\outmjk}{o_{m,j,k}}
\newcommand{\outmcd}{o_{m,c,d}}
\newcommand{\inni}{\iota_{n,i}}
\newcommand{\inna}{\iota_{n,a}}
\newcommand{\innl}{\iota_{n,l}}
\newcommand{\parad}{\shortdfibto}
\newcommand{\paradr}{\shortdfibto}
\newcommand{\paradl}{\shortdfibot}
\newcommand{\xparato}[1]{
  \mathbin{\tikz[baseline] \draw (0pt,.5ex) edge[dfib] node[inner sep=0.5pt,anchor=south,pos=.3] {$\scriptscriptstyle #1$} 
    (1.5ex,.5ex);}}
\newcommand{\xparaot}[1]{
  \mathbin{\tikz[baseline] \draw (1.5ex,.5ex) edge[dfib] node[inner sep=0.5pt,anchor=south,pos=.3] {$\scriptscriptstyle #1$} 
    (0pt,.5ex);}}

\newcommand{\paraer}{\xparato{1}}
\newcommand{\parael}{\xparaot{1}}
\newcommand{\parair}{\xparato{0}}
\newcommand{\parail}{\xparaot{0}}
\newcommand{\synchror}{\shortrightarrow}
\newcommand{\synchrol}{\shortleftarrow}
\newcommand{\synchro}{\shortleftrightarrow}
\newcommand{\untype}{\mathrm{untype}}
\newcommand{\picalclocal}{\picalc_{\mathrm{l}}}
\newcommand{\chilocal}{\chi_{\mathrm{l}}}
\newcommand{\chilocalS}{\chi_{\mathrm{l}}^{\mathrm{S}}}
\DeclareMathOperator{\corelab}{\mathrm{label}}
\newcommand{\colle}[2]{#1 \parallel #2}
\newcommand{\collefun}{{\parallel}}
\newcommand{\poright}[1]{\mathbin{{\triangleright}_{#1}}}
\newcommand{\poleft}[1]{\mathbin{{\triangleleft}_{#1}}}
\newcommand{\posym}[1]{\mathbin{{\diamond}_{#1}}}
\newcommand{\cospanof}[1]{\langle #1 \rangle}

% \newcommand{\rightdpbkblackrev}{\mathbin{\RightDiamond}} *)
% \newcommand{\leftdpbkblackrev}{\mathbin{\rotatebox[origin=c]{180}{$\SmallRightDiamond$}}} *)
\newcommand{\dpbklrev}{\mathbin{\smalltriangleleft\!\!\blacktriangleright}} 
\newcommand{\dpbkrrev}{\mathbin{\blacktriangleleft\!\!\smalltriangleright}} 
\newcommand{\dpbkr}{\mathbin{\blacktriangleright}}
\newcommand{\dpbkl}{\mathbin{\blacktriangleleft}}
\newcommand{\runion}{\mathbin{\sqcup}}
\newcommand{\econt}[2]{#1 \langle #2 \rangle}
\newcommand{\econtii}[2]{#1 {\langle\!\langle} #2 {\rangle\!\rangle}}
%\newcommand{\delocal}{\mathbin{\centerdot}}
\newcommand{\delocaldom}{\mathbin{\square}}
\newcommand{\delocaldomdom}{\mathbin{\smalltriangleup}}
%\newcommand{\bareactions}{\bigcat{actions}}
%\newcommand{\bareaction}[1]{\lfloor #1 \rfloor}
\newcommand{\bareactions}{\B}
\newcommand{\bareaction}[1]{#1}
\newcommand{\etiquette}[1]{\lfloor #1 \rfloor}

\newcommand{\veca}{\vv{a}}
\newcommand{\vdashas}{\mathrel{\vdash_{\veca}}}
\newcommand{\nvdashas}{\mathrel{\nvdash_{\veca}}}
\newcommand{\vdashask}{\mathrel{\vdash_{\veca[k]}}}
\newcommand{\nvdashask}{\mathrel{\nvdash_{\veca[k]}}}
\newcommand{\delocalas}{\mathbin{\centerdot_{\veca}}}
\newcommand{\delocaldomas}{\mathbin{\square_{\veca}}}
\newcommand{\delocaldomdomas}{\mathbin{\smalltriangleup_{\veca}}}
\newcommand{\delocal}[1]{\mathbin{\centerdot_{#1}}}
\newcommand{\delocale}{\delocal{e}}
\newcommand{\delocaldome}{\mathbin{\square_{e}}}
\newcommand{\delocaldomdome}{\mathbin{\smalltriangleup_{e}}}


\newcommand{\vecb}{\vec{b}}
\newcommand{\vdashbs}{\mathrel{\vdash_{\vecb}}}
\newcommand{\nvdashbs}{\mathrel{\nvdash_{\vecb}}}
\newcommand{\vdashbsk}{\mathrel{\vdash_{\vecb[k]}}}
\newcommand{\nvdashbsk}{\mathrel{\nvdash_{\vecb[k]}}}
\newcommand{\delocalbs}{\mathbin{\centerdot_{\vecb}}}
\newcommand{\delocaldombs}{\mathbin{\square_{\vecb}}}
\newcommand{\delocaldomdombs}{\mathbin{\smalltriangleup_{\vecb}}}

\newcommand{\vecc}{\vec{c}}
\newcommand{\vdashcs}{\mathrel{\vdash_{\vecc}}}
\newcommand{\nvdashcs}{\mathrel{\nvdash_{\vecc}}}
\newcommand{\vdashcsk}{\mathrel{\vdash_{\vecc[k]}}}
\newcommand{\nvdashcsk}{\mathrel{\nvdash_{\vecc[k]}}}
\newcommand{\delocalcs}{\mathcin{\centerdot}_{\vecc}}
\newcommand{\delocaldomcs}{\mathbin{\square_{\vecc}}}
\newcommand{\delocaldomdomcs}{\mathbin{\smalltriangleup_{\vecc}}}

\newcommand{\vecd}{\vec{d}}
\newcommand{\vdashds}{\mathrel{\vdash_{\vecd}}}
\newcommand{\nvdashds}{\mathrel{\nvdash_{\vecd}}}
\newcommand{\vdashdsk}{\mathrel{\vdash_{\vecd[k]}}}
\newcommand{\nvdashdsk}{\mathrel{\nvdash_{\vecd[k]}}}
\newcommand{\delocalds}{\mathdin{\centerdot}_{\vecd}}
\newcommand{\delocaldomds}{\mathbin{\square_{\vecd}}}
\newcommand{\delocaldomdomds}{\mathbin{\smalltriangleup_{\vecd}}}

\newcommand{\EqRel}{\mathrm{EqRel}}
\newcommand{\pbkcomplexists}[2]{#1 \drsh #2}
\newcommand{\nombre}[2]{N^{#1}_{#2}}
\newcommand{\incarddom}[2]{#2 \in \carddom(#1)}
\DeclareMathOperator{\carddom}{ep}
\DeclareMathOperator{\ep}{ep}
\newcommand{\mkh}{\Del \xto{h} \Gam}
\newcommand{\mkhi}{\Del' \xto{h'} \Gam'}
\newcommand{\mkhii}{\Del'' \xto{h''} \Gam''}
%\newcommand{\insere}[2]{\mathit{ins}_{#1}^{#2}}
\newcommand{\insere}[2]{{#1} \rightsquigarrow {#2}}
\newcommand{\identify}[2]{{#1} \triangleright {#2}}
\DeclareMathOperator{\fc}{fc}
\DeclareMathOperator{\fmc}{fmc}
\DeclareMathOperator{\fm}{fm}
\DeclareMathOperator{\bc}{bc}
\newcommand{\NProc}{\mathit{NPi}}
\newcommand{\aaand}{\and \mbox{and} \and}
\newcommand{\seq}{\mathbin{;}}
\newcommand{\xxot}[2]{\mathrel{{}_{#1}\!\xot{#2}}}
\newcommand{\xxOt}[2]{\mathrel{{}_{#1}\!\xOt{#2}}}
\newcommand{\relR}{\mathrel{R}}
\newcommand{\relRi}{\mathrel{R'}}
\newcommand{\relRRR}{\mathrel{\RRR}}
\newcommand{\converse}[1]{#1^{\dagger}}
\newcommand{\projLLLlocal}{p^{\LLLlocal}}
\newcommand{\projAR}{p^{\A\R}}
\newcommand{\derivrest}[3]{\restr{(#1 \cdot #2)}{#3}}
\newcommand{\zetabar}{\bar{\zeta}}
\newcommand{\extendn}[2]{\vecteurn{#1}, #2}
\newcommand{\forkln}{\pi^l_n}
\newcommand{\forklp}{\pi^l_p}
\newcommand{\forkrn}{\pi^r_n}
\newcommand{\forkrp}{\pi^r_p}
\newcommand{\forkof}[1]{\pi_{#1}}
\newcommand{\forklof}[1]{\pi^l_{#1}}
\newcommand{\forkrof}[1]{\pi^r_{#1}}
\newcommand{\forkn}{\forkof{n}}
\newcommand{\forkp}{\forkof{p}}

% Labels
\newcommand{\marklabl}[1]{#1}
\newcommand{\labnuout}[2]{\marklabl{[\nu.{#2{!}{-}}]^{#1}}}
\newcommand{\labout}[3]{\marklabl{[#2{!}#3]^{#1}}}
\newcommand{\labin}[2]{\marklabl{[#2{?}]^{#1}}}
\newcommand{\labinknown}[3]{\marklabl{[#2{?}#3]^{#1}}}
\newcommand{\labtau}[1]{\marklabl{[\tau]^{#1}}}
\newcommand{\labl}{v}
\newcommand{\lablb}{w}
\newcommand{\lableq}{\equiv}

\newcommand{\inn}{\mathsf{in}}
\newcommand{\outt}{\mathsf{out}}
\newcommand{\tauu}{\mathsf{tau}}
\newcommand{\ress}{\mathsf{res}}
\newcommand{\paraa}{\mathsf{para}}

% Cells
\newcommand{\incell}[2]{\mathsf{in}_{#1,#2}}
\newcommand{\incellknown}[3]{\mathsf{in}_{#1,#2,#3}}
\newcommand{\outcell}[3]{\mathsf{out}_{#1,#2,#3}}
\newcommand{\opencell}[2]{\mathsf{open}_{#1,#2}}
\newcommand{\closecell}[2]{\mathsf{close}^l_{#1,#2}}
\newcommand{\closelcell}[2]{\closecell{#1}{#2}}
\newcommand{\closercell}[2]{\mathsf{close}^r_{#1,#2}}
\newcommand{\taucell}[3]{\mathsf{tau}^l_{#1,#2,#3}}
\newcommand{\taurcell}[3]{\mathsf{tau}^r_{#1,#2,#3}}
\newcommand{\pararcell}[2]{\mathsf{para}^r_{#1,#2}}
\newcommand{\paralcell}[2]{\mathsf{para}^l_{#1,#2}}
\newcommand{\rescell}[2]{\mathsf{res}_{#1,#2}}
\newcommand{\repcell}[1]{\mathsf{rep}_{#1}}
\newcommand{\permcell}[1]{\mathsf{perm}_{#1}}

% Smart Cells
\newcommand{\sincell}{\mathsf{in}}
\newcommand{\soutcell}{\mathsf{out}}
\newcommand{\sopencell}{\mathsf{open}}
\newcommand{\sclosecell}{\mathsf{close}}
\newcommand{\scloselcell}{\mathsf{close}^l}
\newcommand{\sclosercell}{\mathsf{close}^r}
\newcommand{\staucell}{\mathsf{tau}}
\newcommand{\staulcell}{\mathsf{tau}^l}
\newcommand{\staurcell}{\mathsf{tau}^r}
\newcommand{\spararcell}{\mathsf{para}^r}
\newcommand{\sparalcell}{\mathsf{para}^l}
\newcommand{\srescell}{\mathsf{res}}
\newcommand{\srepcell}{\mathsf{rep}}
\newcommand{\sdupcell}{\mathsf{dup}}
\newcommand{\sfactcell}{\mathsf{fact}}


\newcommand{\vlabtau}{\marklabl{\tau}}
\newcommand{\vlabnuout}{\labnuout{}}
\newcommand{\vlabout}{\labout{}{}}
\newcommand{\vlabin}{\labin{}}
\newcommand{\Sigi}{\bigcat{Sig}_1} %{\bigfun{S}}
\newcommand{\Sigh}{\bigcat{Sig}_h} %{\bigfun{S}}
\newcommand{\Sigv}{\bigcat{Sig}_v} %{\bigfun{S}}
\newcommand{\Sighv}{\bigcat{Sig}_{hv}} %{\bigfun{S}}
% \newcommand{\inop}{\mathsf{in}}
\newcommand{\inop}[1]{#1{?}}
%\newcommand{\outop}{\mathsf{out}}
\newcommand{\outop}[2]{{#1}{!}{#2}}
\newcommand{\newop}{\mathsf{new}}
\newcommand{\paraop}{\mathsf{para}}
\newcommand{\zeroop}{\mathsf{zero}}
\newcommand{\bangop}{\mathsf{bang}}
\newcommand{\cellin}[1]{#1{?}}
\newcommand{\vin}{\cellin{}}
\newcommand{\cellout}[2]{{#1}{!}{#2}}
\newcommand{\vout}{\cellout{}{}}
\newcommand{\celloutnu}[3]{#1 \vdash \nu_{{#2}{!}}}
\newcommand{\voutnu}[1]{\nu_{\cellout{}{}} #1}
\newcommand{\vtau}[2]{\tau(#1,#2)}
\newcommand{\celltau}[2]{\tau({#1},{#2})}
\newcommand{\vtaunu}[2]{\tau_\nu(#1,#2)}
\newcommand{\celltaunu}[2]{\tau_\nu({#1},{#2})}



% \newcommand{\labnuout}[1]{\underline{\nu \overline{#1}}}
% \newcommand{\vlabnuout}{\labnuout{\cdot}}
% \newcommand{\labout}[2]{\underline{\overline{#1} \langle #2 \rangle}}
% \newcommand{\vlabout}{\labout{\cdot}{\cdot}}
% \newcommand{\labin}[1]{\underline{#1}}
% \newcommand{\vlabin}{\labin{\cdot}}
% \newcommand{\Sigi}{\bigcat{Sig}_1} %{\bigfun{S}}
% \newcommand{\inop}{\mathsf{in}}
% \newcommand{\outop}{\mathsf{out}}
% \newcommand{\newop}{\mathsf{new}}
% \newcommand{\paraop}{\mathsf{para}}
% \newcommand{\zeroop}{\mathsf{zero}}
% \newcommand{\vin}{\cdot}
% \newcommand{\cellin}[1]{#1}
% \newcommand{\cellout}[2]{\overline{#1}\tupling{#2}}
% \newcommand{\vout}{\cellout{\cdot}{\cdot}}

\newcommand{\elements}{{\textstyle \int}}
\newcommand{\plays}{\T}
\newcommand{\views}{\V}
\newcommand{\Plays}{\T}
\newcommand{\Views}{\V}
\newcommand{\horizontal}{\bigfun{H}}
\newcommand{\vertical}{\bigfun{V}}
\newcommand{\trasse}{u}

\newcommand{\mumall}{\ensuremath{\mu\mathrm{MALL}}}
\newcommand{\muall}{\ensuremath{\mu\mathrm{ALL}}}
\newcommand{\LLLL}{\mathfrak{L}}
\newcommand{\RRRR}{\mathfrak{R}}
\newcommand{\NNNN}{\mathfrak{N}}
\DeclareMathOperator{\Id}{Id}
\newcommand{\Rtimes}{\mathrm{R}{\times}}
\newcommand{\Lplus}{\mathrm{L}{+}}
\newcommand{\premise}[1]{\mathbf{v}_{#1}}
\newcommand{\positive}{\mathbf{p}}
\newcommand{\negative}{\mathbf{n}}
\newcommand{\cutelim}[2]{[#1 | #2]}
\newcommand{\complementary}[2]{#1 \coh #2}
\newcommand{\flow}[1]{\mathbf{flow}(#1)}
\newcommand{\Flow}[3]{\mathbf{ins}_{#1,#2}(#3)}
\newcommand{\Flowfun}{\mathbf{ins}}
\newcommand{\inactivet}[1]{\mathbf{i}^{\mathit{t}}_{#1}}
\newcommand{\inactives}[1]{\mathbf{i}^{\mathit{s}}_{#1}}
\newcommand{\inserer}[3]{\mathbf{ins}_{#1,#2}(#3)}
\newcommand{\Tens}{\textsc{Tens}\xspace}
\newcommand{\Par}{\textsc{Par}\xspace}
\newcommand{\Plus}{\textsc{Plus}\xspace}
\newcommand{\Plusi}{\textsc{Plus1}\xspace}
\newcommand{\Plusii}{\textsc{Plus2}\xspace}
\newcommand{\With}{\textsc{With}\xspace}
\newcommand{\One}{\textsc{One}\xspace}
\newcommand{\Baut}{\textsc{Bot}\xspace}
\newcommand{\Taupe}{\textsc{Top}\xspace}
\newcommand{\Ax}{\textsc{Ax}\xspace}
\newcommand{\Cut}{\textsc{Cut}\xspace}
\newcommand{\Mu}{\textsc{Mu}\xspace}
\newcommand{\Nu}{\textsc{Nu}\xspace}

\newcommand{\inferr}[3][]{\fbox{\inferrule[#1]{#2}{#3}}}
\newcommand{\tgam}{t^\Gam}
\newcommand{\tdel}{t^\Del}
\newcommand{\tcgam}{(t^c)^\Gam}
\newcommand{\tgamc}{t^{\Gam \times c}}
\newcommand{\tdelgam}{(t^\Del)^\Gam}
\newcommand{\tgamdel}{t^{\Gam \times \Del}}
\newcommand{\vise}[1]{{#1}^{\bullet}}
\newcommand{\pvise}[1]{{#1}^{\rond}}
\newcommand{\viseop}[1]{{#1}_{\bullet}}
\newcommand{\viseopcell}[1]{\mathsf{comp}_{\bullet}(#1)}

% \newcommand{\dcell}[5]{
% %                           1 2 3 4 5   
%   \def\ArgI{#1}%
%   \def\ArgII{#2}%
%   \def\ArgIII{#3}%
%   \def\ArgIV{#4}%
%   \def\ArgV{#5}%
%   \dcellrelay %
% }
% %\NewDocumentCommand{\dcellrelay}{O{} m O{} m O{} m  O{} O{} m}{
% \newcommand{\dcellrelay}[9]{
% %                                6   7  8  9 10  11 12  13  14
%     \diag{%
%       |(X)| {\ArgI} \& |(Y)| {\ArgII} \\ %
%       |(U)| {\ArgIII} \& |(V)| {\ArgIV} %
%     }{%
%       (X) edge[labelu={#1},\ArgV] (Y) %
%       edge[twol={#3},#2] (U) %
%       (Y) edge[twor={#5},#4] (V) %
%       (U) edge[labeld={#7},#6] (V) %
%       (l) edge[cell=.4,labelu={\scriptstyle #9},#8] (r) %
%     }
% }

\newcommand{\constapp}[2]{#1 \llparenthesis #2 \rrparenthesis}
\newcommand{\ruleapp}[2]{#1 \langlebar #2 \ranglebar}
\newcommand{\squares}[1]{#1_{\Box}}
\newcommand{\vcompo}[4][]{(#2).(#3 \vcomp{#1} #4)}
\newcommand{\vmatch}[3]{\vv{#1} \triangleright \vv{#2},\vv{#3}}
\newcommand{\vtarg}{t'}
\DeclareMathOperator{\topb}{\mathsf{t}}
\DeclareMathOperator{\botb}{\mathsf{b}}
\DeclareMathOperator{\rigb}{\mathsf{r}}
\DeclareMathOperator{\lefb}{\mathsf{l}}
\DeclareMathOperator{\fvars}{fv}
\DeclareMathOperator{\ftvars}{ftv}
\tikzset{port/.style={draw,thick,-}}
\newcommand{\colontrans}{\mathrel{:}}
\DeclareMathOperator{\idm}{\id}


==> stacey.tex <==


\makeatletter
\pgfkeys{
  /pgf/scalable arrows/.code={
    \let\pgf@add@arrows@as@needed=\pgf@add@scalable@arrows@as@needed
    \let\pgf@shorten@path@as@needed=\pgf@shorten@path@as@needed@for@scalable
  },
  /pgf/arrow scale factor/.initial=1,
}

\def\pgf@add@scalable@arrows@as@needed{%
  \pgfkeysgetvalue{/pgf/arrow scale factor}{\pgf@temp}%
  \let\pgf@restorelw=\pgfutil@empty
  \ifx\pgf@temp\pgfutil@empty
  \else
  \edef\pgf@restorelw{\noexpand\pgfsetlinewidth{\the\pgflinewidth}}%
  \pgfsetlinewidth{\pgf@temp\pgflinewidth}%
  \fi
  \ifx\pgf@startarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondonpath}{\pgfpointfirstonpath}}
      {\pgf@startarrow}%
  \fi%
  \ifx\pgf@endarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondlastonpath}{\pgfpointlastonpath}}
      {\pgf@endarrow}%
  \fi%
      \pgf@restorelw%
}

\def\pgf@shorten@path@as@needed@for@scalable{%
  \pgfkeysgetvalue{/pgf/arrow scale factor}{\pgf@temp}%
  \let\pgf@restorelw=\pgfutil@empty
  \ifx\pgf@temp\pgfutil@empty
  \else
  \edef\pgf@restorelw{\noexpand\pgfsetlinewidth{\the\pgflinewidth}}%
  \pgfsetlinewidth{\pgf@temp\pgflinewidth}%
  \fi
  \pgfprocesspathextractpoints{\pgf@arrowpath}%
  \let\pgf@arrow@next=\pgf@shorten@now%
  \ifx\pgf@shorten@start\pgfutil@empty%
    \ifx\pgf@shorten@end\pgfutil@empty%
      \ifdim\pgf@shorten@end@additional=0pt\relax%
        \ifdim\pgf@shorten@start@additional=0pt\relax%
          \let\pgf@arrow@next=\relax%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgf@arrow@next%
  \pgf@restorelw%
}

\makeatother

==> tikzlibraryarrows.new.code.tex <==
\usepgflibrary{arrows.new}

\endinput
